TARZAN: A Region-Based Library for Forward and Backward Reachability of Timed Automata (Extended Version)

The zone abstraction, widely adopted for its notable practical efficiency, is the de facto standard in the verification of Timed Automata (TA). Nonetheless, region-based abstractions have been shown to outperform zones in specific subclasses of TA. To complement and support mature zone-based tools, we introduce TARZAN, a C++ region-based verification library for TA. The algorithms implemented in TARZAN use a novel region abstraction that tracks the order in which clocks become unbounded. This additional ordering induces a finer partitioning of the state space, enabling backward algorithms to avoid the combinatorial explosion associated with enumerating all ordered partitions of unbounded clocks, when computing immediate delay predecessor regions. We validate TARZAN by comparing forward reachability results against the state-of-the-art tools Uppaal and TChecker. The experiments confirm that zones excel when TA have large constants and strict guards. In contrast, TARZAN exhibits superior performance on closed TA and TA with punctual guards. Finally, we demonstrate the efficacy of our backward algorithms, establishing a foundation for region-based analysis in domains like Timed Games, where backward exploration is essential.

==> Data_Structure/backup_algorithm/delay_successor_algorithm_backup.tex <==
\begin{algorithm}[tb]
    \caption{\texttt{find-delay-successor}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region.}
    \KwResult{The delay successor of $\reg$.}
    \Begin() {
        $\breg \gets$ copy of $\reg$\;
        
        \uIf{$(p_{\reg} = 0 \land X_{\reg,0} \neq \varnothing) \lor (p_{\reg} > 0 \land X_{\reg,0} \neq \varnothing$)}{
            \texttt{delay-successor-A}$(\breg)$\;
            }
        \ElseIf{$p_{\reg > 0} \land \mathit{X_{\reg,0}} = \varnothing$}{ 
                \texttt{delay-successor-B}$(\breg)$\;
            }
        
        \Return $\breg$\;
        }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-A}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class A.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
            create empty set $X_{\mathit{tmp}}$\;
            create empty set $X_{\mathit{oob}}$\;
            
            \ForEach{$x \in X_{\reg,0}$}{
                \uIf{$h_{\reg}(x) = c_{\max}$}{
                    $X_\mathit{oob} \gets X_\mathit{oob} \cup \{x\}$\;
                }
                \Else{
                    $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{x\}$\;
                }
                $X_{\reg,0} \gets X_{\reg,0} \setminus \{x\}$\;
            }
            
            \If{$X_{\mathit{tmp}} \neq \varnothing$}{
                \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, 0)$\;
            }
            \If{$X_{\mathit{oob}} \neq \varnothing$}{
                \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
            }
    }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-B}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class B.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
           \ForEach{$x \in \mathit{X_{\reg, p}}$}{
                    $h_{\reg}(x) \gets h_{\reg}(x) + 1$\;
                    $X_{\reg,0} \gets X_{\reg,0} \cup \{x\}$\;
                }
           \texttt{remove}$(\reg, p_{\reg})$\;
    }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-C}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class C.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
                create empty set $X_{\mathit{tmp}}$\;
                create empty set $X_{\mathit{oob}}$\;
                
                
                %\For{$i = (p_{\reg} - 1)$ \KwTo $1$}{
                %    \ForEach{$x \in X_{\reg,i}$}{
                %        $X_{\reg,i+1} \gets X_{\reg,i+1} \cup \{x\}$\;
                %        $X_{\reg,i} \gets X_{\reg,i} \setminus \{x\}$\;
                %    }
                %}
                
                \ForEach{$x \in X_{\reg,0}$}{
                    \uIf{$h_{\reg}(x) = c_{\max}$}{
                        $\mathit{X_{oob}} \gets \mathit{X_{oob}} \cup \{x\}$\;
                    }
                    \Else{
                        $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{x\}$\;
                    }
                    $X_{\reg,0} \gets X_{\reg, 0} \setminus \{x\}$\;
                }

                \If{$X_{\mathit{tmp}} \neq \varnothing$}{
                    \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, 0)$\;
                }
                
                \If{$X_{\mathit{oob}} \neq \varnothing$}{
                    \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
                }
    }
\end{algorithm}

==> Data_Structure/transition_classes.tex <==
% Add horizontal padding (extra space between columns)
%\setlength{\tabcolsep}{10pt}
%
% \begin{table}[b]
% \centering
% \renewcommand{\arraystretch}{1.3} % more vertical space
% \begin{tabular}{>{\bfseries}c | c c c c}
% \toprule
%      & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{U} \\
% \midrule
% A & F & T & F & T \\
% B & T & F & T & F \\
% C & F & T & F & F \\
% U & F & F & F & F \\
% \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Transitioning between different classes.}
% \label{tab:transitioning_classes}
% \end{table}
%
%
\begin{figure}[tb]
\centering
\begin{tikzpicture}[
    ->,
    >=stealth',
    shorten >=2pt, 
    auto,
    align=center,
    transform shape,
    line width=1pt
]

% Nodes
\node[state] (A) at (0, 0) {\large{\textbf{A}}};
\node[state] (B) at (3, 0) {\large{\textbf{B}}};
\node[state] (C) at (6, 0) {\large{\textbf{C}}};
\node[state] (U) at (-3, 0) {\large{\textbf{U}}};

% Edges with curved double arrows
\draw[bend left=20, thick] (B) to node[above] {} (A);  
\draw[bend left=20, thick] (A) to node[below] {} (B);  

\draw[bend left=20, thick] (C) to node[right] {} (B);  
\draw[bend left=20, thick] (B) to node[left] {} (C);  

\draw[thick] (A) -- node[left] {} (U);  

\end{tikzpicture}
\caption{The possible ways to transition between classes when using delay transitions.}
\label{fig:dependency_classes}
\end{figure}

==> DelayAndDiscretePredecessors/Delay_Predecessors/Backup_Algorithms/backup.tex <==
\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors}$(\reg)$}
    
    \KwData{$\reg = \{ \loc, h,  X_{-q}, \dots, X_{-1}, X_{0}, X_1, \dots, X_{p} \}$: a region.}
    \KwResult{The delay predecessors of $\reg$.}
    \Begin() {
        create empty set $\res$\;
        \uIf{$p_{\reg} = 0 \land X_{\reg,0} = \varnothing$}{
            $\breg \gets$ copy of $\reg$\;
            \texttt{insert-and-remove-set}$(\breg, -q_{\breg}, 0)$\;
            $\res \gets \res \cup \{ \breg \}$\;
        }
        
        \uElseIf{$p_{\reg} = 0 \land X_{\reg,0} \neq \varnothing$}{
            $\res \gets \res \cup \texttt{delay-predecessors-A-C}(\reg)$\;
        }

        \Else{
            \uIf{$\mathit{X_{\breg,0}} = \varnothing$}{ 
                $\res \gets \res \cup \texttt{delay-predecessors-B}(\reg)$\;
            }
            \Else{
                 $\res \gets \res \cup \texttt{delay-predecessors-A-C}(\reg)$\;
            }
        }
        
        \Return $\res$\;
    }
\end{algorithm}



%\begin{algorithm}[t]
%    \caption{\texttt{delay-predecessors-U}$(\reg)$}
%    \label{alg:finddelaypred}
    
%    \KwData{$\reg$: a region of class U.}
%    \KwResult{The delay predecessors of $\reg$.}
    
%    \Begin() {    
%        $\breg \gets$ copy of $\reg$\;
%        \texttt{insert-and-remove-set}$(\breg, -q_{\breg}, 0)$\;
        %\ForEach{$x \in X_{\breg,-q_{\breg}}$}{
        %    $X_{\breg,0} \gets X_{\breg,0} \cup \{ x \}$\;
        %}
        %\texttt{remove}$(\breg, -q_{\breg})$\;
        \Return $\{ \breg \}$\;
%    }
%\end{algorithm}



\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors-B}$(\reg)$}

    \KwData{$\reg$: a region of class B}
    \KwResult{The delay predecessors of $\reg$.}
    
    \Begin() {
        create empty set $\res$\;
        % È inutile avere la distinzione tra il caso in cui p = 1 e p > 1, siccome il meccanismo usato per tornare indietro è lo stesso. Lascio commentato il secondo branch per completezza.
        %\uIf{$p_{\reg} = 1$}{
            % Case (i A)
            $\breg \gets$ copy of $\reg$\;
            \texttt{insert-and-remove-set}$(\breg, 1, 0)$\;
            $\res \gets \res \cup \{ \breg \}$\;

            % Case (ii A)
            % Questo if ci permette di evitare il calcolo quando siamo in una regione bounded.
            \If{$q_{\reg} \ge 1$}{
                $\breg_1 \gets$ copy of $\reg$\;
                % Possiamo già calcolare il caso C quando p = 1
                \texttt{insert-and-remove-set}$(\breg_1, -q_{\breg_1}, 0)$\;
                $\breg_2 \gets$ copy of $\breg_1$\;
                \texttt{insert-and-remove-set}$(\breg_2, 1, 0)$\;
                $\res \gets \res \cup \{ \breg_1, \breg_2 \}$\;
             }
        %}
        %\Else{
            % Case (i C)
        %    $\breg \gets$ copy of $\reg$\;
        %    \texttt{insert-and-remove-set}$(\breg, 1, 0)$\;
        %    $\res \gets \res \cup \{ \breg \}$\;

            % Case (ii C)
        %    \If{$q_{\reg} \ge 1$}{
        %       $\breg_1 \gets$ copy of $\reg$\;
               % Possiamo già calcolare il caso (iii C) 
        %       \texttt{insert-and-remove-set}$(\breg_1, -q_{\breg_1}, 0)$\;
        %       $\breg_2 \gets$ copy of $\breg_1$\;
        %       \texttt{insert-and-remove-set}$(\breg_2, 1, 0)$\;
        %       $\res \gets \res \cup \{ \breg_1, \breg_2 \}$\;
        %    }
        %}    
        \Return $\res$\;
    }
\end{algorithm}



\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors-A-C}$(\reg)$}
    
    \KwData{$\reg$: a region of either class A or class C.}
    \KwResult{The delay predecessors of $\reg$.}
    
    \Begin() {    
        $\breg \gets$ copy of $\reg$\;
        create empty set $X_{\mathit{tmp}}$\;
        \ForEach{$x \in X_{\breg,0}$}{
            $h_{\breg}(x) \gets h_{\breg}(x) - 1$\;
            $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{ x \}$\;
            $X_{\breg,0} \gets X_{\breg,0} \setminus x$\;
        }
        \texttt{insert-right}$(\breg, X_{\mathit{tmp}}, p_{\breg})$\;
        \Return $\{ \breg \}$\;
    }
\end{algorithm}
%\todoAM{}{Nell'algoritmo A e C, mettere $p_{\breg}$ va bene perchè se R è ri classe A allora p è 0, altrimenti p è maggiore di 0 e i clock vengono inseriti in fondo alla lista di quelli con parte frazionaria maggiore di 0.}
%
%
%
%
%%%%
%% ANDREBBERO INSERITI DEI SIDE CHECKS CHE CONTROLLANO CHE IL VALORE INTERO DEI CLOCK SIA MAGGIORE DI 0
%%%%
%% SE METTI H CAMBIA FONT METTENDOLO PIÙ GRANDE DI QUANDO USI tb
%%%%
%
% create empty set $X_{\mathit{tmp}}$\;
%                \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, p_{\reg})$\;
%                
%                \For{$i = (p_{\reg} - 1)$ \KwTo $1$}{
%                    \ForEach{$x \in X_{\reg,i}$}{
%                        $X_{\reg,i+1} \gets X_{\reg,i+1} \cup \{x\}$\;
%                        $X_{\reg,i} \gets X_{\reg,i} \setminus \{x\}$\;
%                    }
%                }
%                
%                create empty set $X_{\mathit{oob}}$\;
%                \ForEach{$x \in X_{\reg,0}$}{
%                    \uIf{$h_{\reg}(x) = c_{\max}$}{
%                        $\mathit{X_{oob}} \gets \mathit{X_{oob}} \cup \{x\}$\;
%                    }
%                    \Else{
%                        $X_{\reg,1} \gets X_{\reg,1} \cup \{x\}$\;
%                    }
%                    $X_{\reg,0} \gets X_{\reg, 0} \setminus \{x\}$\;
%                }
%                
%                \If{$X_{\mathit{oob}} \neq \varnothing$}{
%                    \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
%                }
%                
%                \If{$X_{\reg,1} = \varnothing$}{
%                    \texttt{remove}$(\reg, 1)$\;
%                }

==> DelayAndDiscretePredecessors/Discrete_Predecessors/backups/discrete_predecessors_algorithm_backup.tex <==
\begin{algorithm}[tb]
    \caption{\texttt{find-discrete-predecessors}$(\reg)$}

    
    \KwData{$\reg$: a region.}
    \KwResult{The set of regions reachable via backward discrete transitions from $\reg$.}
    
    \Begin(){
        $\mathit{res} \gets \varnothing$\;
        
        %\tcp{Get discrete transitions in the original \ac{ta} ending in $\mathit{loc}_{\reg}$}
        $\mathcal{T} \gets \{ (\mathit{loc}', a, \gamma, Y, \mathit{loc}_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, \mathit{loc}' \in Q \}$\;

        \ForEach{$t \in \mathcal{T}$}{
        
        $X_{\mathit{bnd}} \gets \varnothing$\;
        $X_{\mathit{oob}} \gets \varnothing$\;
        
        \ForEach{clock constraint $\ccstr \in \gamma$}{
            $\breg \gets$ copy of $\reg$\;

            \uIf{$(\ccstr{}$ is an equality constraint: $x = c) \land (x \in Y)$}{
                $h_{\breg}(x) = c$\;
            }

            \uElseIf{$(\ccstr{}$ is an inequality constraint: $x > \cmax) \land (x \in Y)$}{
                $X_{\mathit{oob}} \gets X_{\mathit{oob}} \cup \{ x \}$\;
            }

            \ElseIf{$x \in Y$}{
                $X_{\mathit{bnd}} \gets X_{\mathit{bnd}} \cup \{ x \}$\;
            }
        }

        $\mathit{tmp} \gets \varnothing$\;
        $\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
        $\Pi_{\mathit{oob}} \gets $ all partitions of $X_{\mathit{oob}}$\;

        \ForEach{partition $\pi \in \Pi_{\mathit{oob}}$}{
            %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
            $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
            \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                $\mathit{tmp} \gets \mathit{tmp} \cup \{ \breg' \}$\;
            }
        }

        \ForEach{$\mathcal{H} \in \{0, 1, \dots, \cmax + 1\}^{\lvert X_{\mathit{bnd}} \rvert}$}{
            \If{each $x \in X_{\mathit{bnd}}$ can have $h(x)$ according to $\mathcal{H}$ and $\gamma$}{
                $\mathit{tmp}' \gets$ copy of $\mathit{tmp}$\;
                
                \If{some clocks $\Delta \subseteq X_{\mathit{bnd}}$ are unbounded}{

                    \ForEach{$\breg \in \mathit{tmp}$}{

                    $\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
                    $\Pi_{\Delta} \gets $ all partitions of $X_{\Delta}$\;

                    \ForEach{partition $\pi \in \Pi_{\Delta}$}{
                        $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                        \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                            $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                            $\mathit{tmp}' \gets \mathit{tmp}' \cup \{ \breg' \}$\;
                        }
                    }
                    }
                }

                \ForEach{$\breg \in \mathit{tmp}'$}{
                    $\mathcal{X} \gets \{ X_{\breg, 1}, \dots, X_{\breg, p_{\breg}} \}$\;
                    $\Pi_{\mathit{bnd}} \gets $ all partitions of $X_{\mathit{bnd}}$\;

                    \ForEach{partition $\pi \in \Pi_{\mathit{bnd}}$}{
                        $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                       %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                        \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                            $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $o$ and where clocks have an integer value according to $\mathcal{H}$\;
                            $\res \gets \res \cup \{ \breg' \}$\;
                        }
                    }
                }
                
            }
        }
        }

        \Return $\res$\;
    }
\end{algorithm}

\todoAM{}{vedere se tenere questa notazione ed eventualmente adattare il resto prima}

==> DelayAndDiscretePredecessors/Discrete_Predecessors/backups/discrete_predecessors_v2.tex <==
\begin{algorithm}[!hb]
    \caption{\texttt{find-discrete-predecessors}$(\reg)$}

    
    \KwData{$\reg$: a region.}
    \KwResult{The set of regions reachable via backward discrete transitions from $\reg$.}
    
    \Begin(){
        $\mathit{res} \gets \varnothing$\;
        
        %\tcp{Get discrete transitions in the original \ac{ta} ending in $\mathit{loc}_{\reg}$}
        %$\mathcal{T} \gets \{ (\mathit{loc}, a, \gamma, Y, \mathit{loc}_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, \mathit{loc} \in Q \}$\;

        \ForEach{$t \in \{ (q, a, \gamma, Y, q_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, q \in Q \}$}{
        
        $X_{\mathit{bnd}} \gets \varnothing$; $X_{\mathit{oob}} \gets \varnothing$\;
        $\breg \gets$ copy of $\reg$\;
        
        \ForEach{clock constraint $\ccstr \in \gamma$}{

            \uIf{$(\ccstr{}$ is an equality constraint: $x = c) \land (x \in Y)$}{
                $h_{\breg}(x) = c$\;
            }

            \uElseIf{$(\ccstr{}$ is an inequality constraint: $x > \cmax) \land (x \in Y)$}{
                $X_{\mathit{oob}} \gets X_{\mathit{oob}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\;
            }

            \ElseIf{$($clock $x$ appears in $\ccstr) \land (x \in Y)$}{
                $X_{\mathit{bnd}} \gets X_{\mathit{bnd}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\;
            }
        }
        
        %$\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
        %$\Pi_{\mathit{oob}} \gets $ all partitions of $X_{\mathit{oob}}$\;

        %\ForEach{partition $\pi \in \Pi_{\mathit{oob}}$}{
        %    %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
        %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
        %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
        %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
        %        $\mathit{tmp} \gets \mathit{tmp} \cup \{ \breg' \}$\;
        %    }
        %}

        $\mathit{tmp} \gets$ \texttt{perm-regs}($\breg, -q_{\breg}, -1, X_\mathit{oob}, h_{\breg}, \varnothing$)\;

        \ForEach{$h \in \{0, 1, \dots, \cmax + 1\}^{\lvert X_{\mathit{bnd}} \rvert}$}{
            \If{$\forall x \in X_{\mathit{bnd}} : h(x) = h_{\breg}(x)$ and $h$ satisfies $\gamma$}{
                $\mathit{tmp}' \gets$ copy of $\mathit{tmp}$\;
                $\Delta \gets \{ x \in X_{\mathit{bnd}} \; \vert \; h(x) > \cmax \}$\;
                
                \If{$\Delta \neq \varnothing$}{

                    \ForEach{$R \in \mathit{tmp}$}{

                    %$\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
                    %$\Pi_{\Delta} \gets $ all partitions of $X_{\Delta}$\;

                    %\ForEach{partition $\pi \in \Pi_{\Delta}$}{
                    %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                    %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                    %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                    %        $\mathit{tmp}' \gets \mathit{tmp}' \cup \{ \breg' \}$\;
                    %    }
                    $\mathit{tmp}' \gets \mathit{tmp}'$ $\cup$ \texttt{perm-regs}($R, -q_R, -1, \Delta, h_R, X_{\mathit{oob}}$)\;
                    }
                }

                \ForEach{$R \in \mathit{tmp}'$}{
                    %$\mathcal{X} \gets \{ X_{\breg, 1}, \dots, X_{\breg, p_{\breg}} \}$\;
                    %$\Pi_{\mathit{bnd}} \gets $ all partitions of $X_{\mathit{bnd}}$\;

                    %\ForEach{partition $\pi \in \Pi_{\mathit{bnd}}$}{
                    %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                       %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                    %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                    %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $o$ and where clocks have an integer value according to $\mathcal{H}$\;
                    %        $\res \gets \res \cup \{ \breg' \}$\;
                    %    }
                    $\res \gets \res$ $\cup$ \texttt{perm-regs}($R, 1, p_R, X_{\mathit{bnd}} \setminus \Delta, h, \varnothing$)\;
                    }
            }

        }
                
        }

        \Return $\res$\;

        \BlankLine
        \BlankLine

        \SetKwFunction{gaop}{perm-regs}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\gaop{$\reg, i, j, X, \mathcal{H}, X_{\mathit{ignore}}$}}{
            $\res \gets \varnothing$\;
            clamp to $\cmax$ all values of $\mathcal{H}$ that are greater than $\cmax$\;
            $\mathcal{X} \gets \{ X_{\reg, i}, \dots, X_{\reg, j} \} \setminus X_{\mathit{ignore}}$\;
            $\Pi \gets $ all partitions of $X$\;

            \ForEach{partition $\pi \in \Pi$}{
                $\mathcal{Z} \gets$ all permutations of ($\mathcal{X} \cup \pi$) that preserve the order of $\mathcal{X}$\;
                %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                   $\breg \gets $ copy of $\reg$ such that (i) sets ($\mathcal{X} \cup \pi$) are reordered according to $\zeta$ and (ii) clocks have a value given by $\mathcal{H}$\;
                   $\res \gets \res \cup \{ \breg \}$\;
                }
           }
           \Return $\res$\;
        }        
    }
\end{algorithm}

\todoAM{}{Cambiare in tutto il paper l'indice $q$ con $\ell$ e $p$ con $r$ OKKIO anche al teorema 2}

==> DelayAndDiscretePredecessors/production_cell.tex <==
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[
	->,
	>=stealth',
	shorten >=2pt, 
	auto,
    transform shape,
    align=center,
    scale=0.77,
    state/.style={thick, circle, draw, minimum size=1.3cm}
    ] 
    
    \node[
          state,
          initial,
          initial text =,
          label=above left:$\mathbf{c}$
         ] 
         (q0) {$\mathit{feed}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          right = 4.6cm of q0
         ] 
         (q1) {$\mathit{table}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          right = 4.6cm of q1
         ] 
         (q2) {$\mathit{robot_p}$};

    \node[
          state,
          label=above left:$\mathbf{c}$,
          above = 2.8cm of q2
         ] 
         (q3) {$\mathit{press}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          left = 4.6cm of q3
         ] 
         (q4) {$\mathit{robot_d}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          left = 4.6cm of q4
         ] 
         (q5) {$\mathit{depot}$};

    \node[
          state,
          label=above left:$\mathbf{e}$,
          left = 0cm of q2,
          yshift=2.7cm
         ] 
         (q6) {$\mathit{fall_p}$};

    \node[
          state,
          label=above left:$\mathbf{e}$,
          right = 0cm of q0,
          yshift=2.7cm
         ] 
         (q7) {$\mathit{fall_d}$};

	\draw [line width=0.35mm] 
    
	(q0) 
    edge 
    node[above, pos=0.6]{$\mathit{toTable}$ \\ $x = 2$} 
    node[below, pos=0.6]{$\resetClock{x}$}
    (q1)
	
    (q1) 
    edge 
    node[above, pos=0.4]{$\mathit{takePlate_p}$ \\ $x \ge 1 \land x \le 3$} 
    node[below, pos=0.4]{$\resetClock{x}$}
    (q2)

    (q2) 
    edge 
    node[right]{$\mathit{toPress}$ \\ $x \ge 2 \land x \le 4$ \\ $\resetClock{x}$}
    (q3)

    (q3) 
    edge 
    node[above]{$\mathit{takePlate_d}$ \\ $x \ge 3 \land x \le 5$} 
    node[below]{$\resetClock{x}$}
    (q4)

    (q4) 
    edge 
    node[above]{$\mathit{toDepot}$ \\ $x \ge 3 \land x \le 6$} 
    node[below]{$\resetClock{x}$}
    (q5)

    (q2) 
    edge 
    node[left, xshift=-9pt]{$\mathit{toPress}$ \\ $x < 2$ \\ $\resetClock{x}$}
    (q6)

    (q4) 
    edge %[out=270, in=0]
    node[right, pos=0.4, xshift = -12pt, yshift=-20pt]{$\mathit{toDepot}$ \\ $x \ge 4$ \\ $\resetClock{x}$}
    (q7)

    (q6) 
    edge [out=180, in=15]
    node[right, pos=0.5, xshift=22pt]{$\mathit{restore_p}$ \\ $x > 1 \land x < 2$}
    (q0)

    (q7) 
    edge
    node[right, pos=0.4, xshift=-2pt]{$\mathit{restore_d}$ \\ $x > 1 \land x \le 5$}
    (q0)

    (q5) 
    edge 
    node[left]{ $\mathit{newPlate}$ \\ $\resetClock{x}$}
    (q0)
	;
\end{tikzpicture}
\end{center}
\caption{A \ac{ta} modeling a Production Cell.
The passage of time is tracked by a clock $y$, which is neither reset nor used in any guard, and is therefore omitted from the figure.}
\label{fig:production_cell_text}
\end{figure}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Conclusion/conclusion.tex <==
We introduced \toolname{}, a region-based verification library supporting forward and backward reachability for \ac{ta}. 
%\toolname{} relies on a refined region abstraction that tracks the order in which clocks become unbounded. 
Our experiments demonstrated that \toolname{} exhibits superior performance on closed \ac{ta} and \ac{ta} with punctual guards, while zone-based approaches remain better suited to other classes of \ac{ta}. 
We showed that backward reachability with \toolname{} is often feasible in practice and effective for verifying safety properties.
\Red{For this reason, the integration of \toolname{} into existing tools has the potential to enhance their verification capabilities.}

Future work will proceed in several directions. 
We plan to integrate additional optimizations into \toolname{}, with a particular focus on improving the computation of delay successors and predecessors, while leveraging symbolic techniques to reduce memory usage. 
In addition, we will extend backward reachability algorithms to networks of \ac{ta}, thereby laying the foundation for applying \toolname{} to the synthesis of winning strategies in Timed Games.
Finally, we intend to explore hybrid approaches that complement \toolname{} with zone-based techniques, thereby combining the strengths of both abstractions.

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Data_Structure/backup_algorithm/delay_successor_algorithm_backup.tex <==
\begin{algorithm}[tb]
    \caption{\texttt{find-delay-successor}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region.}
    \KwResult{The delay successor of $\reg$.}
    \Begin() {
        $\breg \gets$ copy of $\reg$\;
        
        \uIf{$(p_{\reg} = 0 \land X_{\reg,0} \neq \varnothing) \lor (p_{\reg} > 0 \land X_{\reg,0} \neq \varnothing$)}{
            \texttt{delay-successor-A}$(\breg)$\;
            }
        \ElseIf{$p_{\reg > 0} \land \mathit{X_{\reg,0}} = \varnothing$}{ 
                \texttt{delay-successor-B}$(\breg)$\;
            }
        
        \Return $\breg$\;
        }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-A}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class A.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
            create empty set $X_{\mathit{tmp}}$\;
            create empty set $X_{\mathit{oob}}$\;
            
            \ForEach{$x \in X_{\reg,0}$}{
                \uIf{$h_{\reg}(x) = c_{\max}$}{
                    $X_\mathit{oob} \gets X_\mathit{oob} \cup \{x\}$\;
                }
                \Else{
                    $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{x\}$\;
                }
                $X_{\reg,0} \gets X_{\reg,0} \setminus \{x\}$\;
            }
            
            \If{$X_{\mathit{tmp}} \neq \varnothing$}{
                \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, 0)$\;
            }
            \If{$X_{\mathit{oob}} \neq \varnothing$}{
                \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
            }
    }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-B}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class B.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
           \ForEach{$x \in \mathit{X_{\reg, p}}$}{
                    $h_{\reg}(x) \gets h_{\reg}(x) + 1$\;
                    $X_{\reg,0} \gets X_{\reg,0} \cup \{x\}$\;
                }
           \texttt{remove}$(\reg, p_{\reg})$\;
    }
\end{algorithm}

\begin{algorithm}[tb]
    \caption{\texttt{delay-successor-C}$(\reg)$}
    \label{alg:finddelaysucc}
    
    \KwData{$\reg$: a region of class C.}
    \KwResult{\emph{None}, as the changes are applied directly to $\reg$.}
    \Begin() {
                create empty set $X_{\mathit{tmp}}$\;
                create empty set $X_{\mathit{oob}}$\;
                
                
                %\For{$i = (p_{\reg} - 1)$ \KwTo $1$}{
                %    \ForEach{$x \in X_{\reg,i}$}{
                %        $X_{\reg,i+1} \gets X_{\reg,i+1} \cup \{x\}$\;
                %        $X_{\reg,i} \gets X_{\reg,i} \setminus \{x\}$\;
                %    }
                %}
                
                \ForEach{$x \in X_{\reg,0}$}{
                    \uIf{$h_{\reg}(x) = c_{\max}$}{
                        $\mathit{X_{oob}} \gets \mathit{X_{oob}} \cup \{x\}$\;
                    }
                    \Else{
                        $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{x\}$\;
                    }
                    $X_{\reg,0} \gets X_{\reg, 0} \setminus \{x\}$\;
                }

                \If{$X_{\mathit{tmp}} \neq \varnothing$}{
                    \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, 0)$\;
                }
                
                \If{$X_{\mathit{oob}} \neq \varnothing$}{
                    \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
                }
    }
\end{algorithm}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Data_Structure/data_structure.tex <==
We introduce a new region representation that captures the order in which clocks become unbounded (exceeding $\cmax$).
For bounded clocks (with value up to $\cmax$), only the ordering of their fractional part is preserved.
\Red{Our representation builds on~\cite{Bouyer2008}, which focuses on \acp{ta} with bounded clocks.
By also handling unbounded clocks, we significantly extend the applicability of region-based state space exploration to a broader class of \acp{ta}.}
{While forward exploration remains unaffected, our representation influences backward exploration (\autoref{thm:bounded_d_pred} and \autoref{thr:discrete_predecessor_complexity}).}

Let $\aut = (\act, Q, Q_{0}, \ackc, T, \invariant)$ be a \ac{ta}, $q \in Q$.
Furthermore, let $\lidx, \ridx \in \mathbb{N}$ be two integers such that $\lidx + \ridx \le \lvert \ackc \rvert$.
We denote by $X_i \subseteq \ackc$ a subset of clocks of $\aut$, for $-\lidx \le i \le \ridx$.
\Red{We require that these subsets induce a partition of $\ackc$, \emph{i.e.}, $\ackc = \bigcup_{i} X_i$ and, for all indices $-\lidx \le i,j \le \ridx$ such that $i \neq j$, $X_i \cap X_j = \varnothing$.}
Finally, we introduce a function $h : \ackc \rightarrow \{0, \dots, \cmax \}$ that assigns an integer value to each clock in $\ackc$.
%
A region of $\aut$ can be represented as follows:
\begin{equation}
\label{eq:region}
    \reg := \{ \loc, h,  X_{-\lidx}, X_{-(\lidx-1)}, \dots, X_{-1}, X_{0}, X_1, \dots, X_{(\ridx-1)}, X_{\ridx} \}.
\end{equation}
%where $\loc \in Q$ $\loc \in Q$ and $h : \ackc \rightarrow \{0, \dots, \cmax \}$ is a function assigning an integer value to every clock of $\ta$.
%The sets $X_i$ in \autoref{eq:region} form a partition of $\ackc$. %, $-\lidx \le i \le \ridx$. 

Set $X_0$ is always present even if empty; the other sets are omitted when empty.
The sets $X_{-\lidx}, \dots, X_{-1}$ represent unbounded clocks, capturing the ordering in which these clocks become unbounded
(\emph{e.g.}, all clocks in $X_{-1}$ become unbounded simultaneously and prior to all clocks in $X_{-2}$).  
Conversely, the sets $X_1, \dots, X_{\ridx}$ represent bounded clocks, capturing the ordering of their fractional parts (\emph{e.g.}, the fractional parts of all clocks in $X_{1}$ are equal and less than the fractional parts of all clocks in $X_{2}$).
$X_0$ contains bounded clocks that have no fractional part (we also say these clocks \emph{are in the unit}).
The integers $\lidx$ and $\ridx$ denote the number of sets containing unbounded and bounded clocks, respectively ($\ridx$ does not consider $X_0$).  
Their values are automatically updated whenever a set is inserted into or removed from $\reg$.
We use a subscript to disambiguate between different regions: for instance, $q_{\reg}$ refers to the location $q$ of $\reg$, $X_{\reg,0}$ to the set $X_0$ of $\reg$, and $\lidx_{\reg}$ indicates the number of sets containing unbounded clocks in $\reg$.

\Red{For conciseness, we also refer to the elements of a region $\reg$ as its \emph{structure}.
Two regions $\reg,\reg'$ are \emph{structurally equivalent} if the following holds: 
$q_{\reg} = q_{\reg'} 
\land 
%h_{\reg} = h_{\reg'} 
%\land 
\lidx_{\reg} = \lidx_{\reg'}
\land
\ridx_{\reg} = \ridx_{\reg'}$
and, for all $-\lidx_{\reg} \le i \le \ridx_{\reg}$, $X_{\reg, i} = X_{\reg', i}$.}

%To denote all clocks of $\reg$ we also use the following notation:
%$
%\allclocks{\reg} = \bigcup_{i = -\lidx_{\reg}}^{\ridx_{\reg}} X_{\reg, i}
%$.
\begin{example}
\label{ex:exampleregion}
    Let $\aut$ be a \ac{ta} with clocks $\ackc = \{ x, y, z, w \}$ and $\cmax = 5$.
    Consider the region defined as:
    $\{ (x,y,z,w) \; \vert \; 2 < x < 3, 2 < y < 3, z > 5, w > 5, x = y \}$,
    \emph{i.e.}, a region (assumed to be in $q \in Q$) in which $x$ and $y$ are bounded and equal (they have the same fractional part),
    while clocks $z$ and $w$ are unbounded (we assume that $z$ became unbounded before $w$).
    The region is represented using \autoref{eq:region} as:
    $
    \reg = \{ q, h(x) = 2, h(y) = 2, h(z) = 5, h(w) = 5, X_{-2}, X_{-1}, X_0, X_1 \},
    $
    where $X_{-2} = \{ w \}, X_{-1} = \{ z \}, X_0 = \varnothing, X_1 = \{ x, y \}, \lidx = 2$, and $\ridx = 1$.
    
\end{example}

\begin{definition}[Region class]
\label{def:region_classes}
    If the order in which clocks become unbounded is tracked, regions can be classified in four distinct \emph{classes}---\ca{} (Zero), \cb{} (Positive), \cc{} (Mixed), and \cu{} (Unbounded)---defined as:
%\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
    \emph{(i)} Class \ca:~$
    \lidx \ge 0 \land \ridx = 0 \land X_0 \neq \varnothing$;
    %\ca:~$\rega = \{ \loc, h, X_{-\lidx}, \dots, X_{-1}, X_{0} \}: X_0 \neq \varnothing$.
    \emph{(ii)} Class \cb:~$\lidx \ge 0 \land \ridx > 0 \land X_0 = \varnothing$; 
    %$ \land X_1, \dots, X_{\ridx} \neq \varnothing$.
    %\cb:~$\regb = \{ \loc, h, X_{-\lidx}, \dots, X_{-1}, X_{0}, X_1, \dots, X_{\ridx} \} : X_0 = \varnothing \land X_1, \dots, X_{\ridx} \neq \varnothing$.
    \emph{(iii)} Class \cc:~$\lidx \ge 0 \land \ridx > 0 \land X_0 \neq \varnothing$;
    % \land X_1, \dots, X_{\ridx} \neq \varnothing$.
    %\cc:~$\regc = \{  \loc, h, X_{-\lidx}, \dots, X_{-1}, X_{0}, X_1, \dots, X_{\ridx} \} : X_0 \neq \varnothing \land X_1, \dots, X_{\ridx} \neq \varnothing$.
    and \emph{(iv)} Class \cu:~$\lidx > 0 \land \ridx = 0 \land X_0 = \varnothing$.
    % \land X_{-\lidx}, \dots, X_{-1} \neq \varnothing$.
    %\cu:~$\regu = \{  \loc, h, X_{-\lidx}, \dots, X_{-1}, X_{0} \} : X_0 = \varnothing \land X_{-\lidx}, \dots, X_{-1} \neq \varnothing$.
%\end{itemize}
\end{definition}

Class $\ca{}$ denotes regions in which some clocks may be unbounded, while all bounded clocks have no fractional part and at least one clock must be bounded.
Class $\cb{}$ denotes regions where some clocks may be unbounded, and all bounded clocks have a fractional part greater than zero (again, at least one clock must be bounded).
Class $\cc{}$ denotes regions where some clocks may be unbounded and the bounded clocks are partitioned into those with no fractional part and those with a fractional part greater than zero (at least two clocks must be bounded, one with no fractional part and one with a fractional part greater than zero).
Finally, class $\cu{}$ denotes regions in which all clocks are unbounded.
Notice that the region presented in \autoref{ex:exampleregion} belongs to class $\cb$.
This classification into different classes lies at the core of the algorithms that compute the immediate delay successor and immediate delay predecessors of a given region.


\textbf{Transitioning between classes}~Let $\rega$, $\regb$, $\regc$, and $\regu$ be regions of classes $\ca$, $\cb$, $\cc$, and $\cu$, respectively. 
Transitions from a region to its immediate delay successor
induce the following deterministic transitions between classes:%, as shown in \autoref{fig:dependency_classes}.\input{Data Structure/transition_classes}
%
\begin{itemize}[topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt]
    \item \emph{From $\rega$ to $\regb$}: at least one clock $x \in X_{\rega,0}$ must increase such that its fractional part becomes greater than zero, while remaining bounded. 
    Other clocks in $X_{\rega,0}$ can either become unbounded or remain bounded and grow at the same rate of $x$, \emph{i.e.}, all bounded clocks have the same fractional part.
    
    \item \emph{From $\rega$ to $\regu$}: all clocks in $X_{\rega,0}$ become unbounded simultaneously.
    
    \item \emph{From $\regb$ to $\rega$}: it must hold that $\ridx_{\regb} = 1$.
    All clocks in $X_{\regb, 1}$
    must reach the next unit (they will be inserted into $X_{\rega,0}$) and their integer value is incremented by 1, as they have a fractional part greater than zero.

    \item \emph{From $\regb$ to $\regc$}: it must hold that $\ridx_{\regb} > 1$.
    All clocks in $X_{\regb, \ridx_{\regb}}$ must reach the next unit (they will be inserted into $X_{\regc,0}$) and their integer value is incremented by 1, \Red{as they have the biggest fractional part.}

    \item \emph{From $\regc$ to $\regb$}: clocks in $X_{\regc,0}$ can become unbounded or their fractional part can become greater than zero while remaining bounded.
\end{itemize}
The missing transitions between classes are explained as follows.
By \autoref{def:region_classes}, transitioning to $\regu$ is only possible from $\rega$, since $\ridx_{\regu} = 0 \land X_{\regu, 0} = \varnothing$ must hold.
It is not possible to transition from $\rega$ to $\regc$, since all clocks will exit from $X_{\rega, 0}$.
An immediate delay successor of $\regc$ has at least one clock with a nonzero fractional part, making it impossible to transition from $\regc$ to $\rega$.

Transitions between classes contain no self-loops; the immediate delay successor of any region is always a distinct region.
$\regu$ does not have delay successors, as clocks can increase indefinitely once unbounded.
The structure of regions influences transitioning between classes;
\emph{e.g.}, from $\regc$ with $\ridx_{\regc} = 3$, several cycles between $\regb$ and $\regc$ are required before reaching $\rega$ via delay transitions; this becomes possible once $\ridx_{\regc}$ decreases to $1$ as some clocks become unbounded.

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Data_Structure/transition_classes.tex <==
% Add horizontal padding (extra space between columns)
%\setlength{\tabcolsep}{10pt}
%
% \begin{table}[b]
% \centering
% \renewcommand{\arraystretch}{1.3} % more vertical space
% \begin{tabular}{>{\bfseries}c | c c c c}
% \toprule
%      & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{U} \\
% \midrule
% A & F & T & F & T \\
% B & T & F & T & F \\
% C & F & T & F & F \\
% U & F & F & F & F \\
% \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{Transitioning between different classes.}
% \label{tab:transitioning_classes}
% \end{table}
%
%
\begin{figure}[tb]
\centering
\begin{tikzpicture}[
    ->,
    >=stealth',
    shorten >=2pt, 
    auto,
    align=center,
    transform shape,
    line width=1pt
]

% Nodes
\node[state] (A) at (0, 0) {\large{\textbf{A}}};
\node[state] (B) at (3, 0) {\large{\textbf{B}}};
\node[state] (C) at (6, 0) {\large{\textbf{C}}};
\node[state] (U) at (-3, 0) {\large{\textbf{U}}};

% Edges with curved double arrows
\draw[bend left=20, thick] (B) to node[above] {} (A);  
\draw[bend left=20, thick] (A) to node[below] {} (B);  

\draw[bend left=20, thick] (C) to node[right] {} (B);  
\draw[bend left=20, thick] (B) to node[left] {} (C);  

\draw[thick] (A) -- node[left] {} (U);  

\end{tikzpicture}
\caption{The possible ways to transition between classes when using delay transitions.}
\label{fig:dependency_classes}
\end{figure}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Delay_Predecessors/Backup_Algorithms/backup.tex <==
\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors}$(\reg)$}
    
    \KwData{$\reg = \{ \loc, h,  X_{-q}, \dots, X_{-1}, X_{0}, X_1, \dots, X_{p} \}$: a region.}
    \KwResult{The delay predecessors of $\reg$.}
    \Begin() {
        create empty set $\res$\;
        \uIf{$p_{\reg} = 0 \land X_{\reg,0} = \varnothing$}{
            $\breg \gets$ copy of $\reg$\;
            \texttt{insert-and-remove-set}$(\breg, -q_{\breg}, 0)$\;
            $\res \gets \res \cup \{ \breg \}$\;
        }
        
        \uElseIf{$p_{\reg} = 0 \land X_{\reg,0} \neq \varnothing$}{
            $\res \gets \res \cup \texttt{delay-predecessors-A-C}(\reg)$\;
        }

        \Else{
            \uIf{$\mathit{X_{\breg,0}} = \varnothing$}{ 
                $\res \gets \res \cup \texttt{delay-predecessors-B}(\reg)$\;
            }
            \Else{
                 $\res \gets \res \cup \texttt{delay-predecessors-A-C}(\reg)$\;
            }
        }
        
        \Return $\res$\;
    }
\end{algorithm}



%\begin{algorithm}[t]
%    \caption{\texttt{delay-predecessors-U}$(\reg)$}
%    \label{alg:finddelaypred}
    
%    \KwData{$\reg$: a region of class U.}
%    \KwResult{The delay predecessors of $\reg$.}
    
%    \Begin() {    
%        $\breg \gets$ copy of $\reg$\;
%        \texttt{insert-and-remove-set}$(\breg, -q_{\breg}, 0)$\;
        %\ForEach{$x \in X_{\breg,-q_{\breg}}$}{
        %    $X_{\breg,0} \gets X_{\breg,0} \cup \{ x \}$\;
        %}
        %\texttt{remove}$(\breg, -q_{\breg})$\;
        \Return $\{ \breg \}$\;
%    }
%\end{algorithm}



\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors-B}$(\reg)$}

    \KwData{$\reg$: a region of class B}
    \KwResult{The delay predecessors of $\reg$.}
    
    \Begin() {
        create empty set $\res$\;
        % È inutile avere la distinzione tra il caso in cui p = 1 e p > 1, siccome il meccanismo usato per tornare indietro è lo stesso. Lascio commentato il secondo branch per completezza.
        %\uIf{$p_{\reg} = 1$}{
            % Case (i A)
            $\breg \gets$ copy of $\reg$\;
            \texttt{insert-and-remove-set}$(\breg, 1, 0)$\;
            $\res \gets \res \cup \{ \breg \}$\;

            % Case (ii A)
            % Questo if ci permette di evitare il calcolo quando siamo in una regione bounded.
            \If{$q_{\reg} \ge 1$}{
                $\breg_1 \gets$ copy of $\reg$\;
                % Possiamo già calcolare il caso C quando p = 1
                \texttt{insert-and-remove-set}$(\breg_1, -q_{\breg_1}, 0)$\;
                $\breg_2 \gets$ copy of $\breg_1$\;
                \texttt{insert-and-remove-set}$(\breg_2, 1, 0)$\;
                $\res \gets \res \cup \{ \breg_1, \breg_2 \}$\;
             }
        %}
        %\Else{
            % Case (i C)
        %    $\breg \gets$ copy of $\reg$\;
        %    \texttt{insert-and-remove-set}$(\breg, 1, 0)$\;
        %    $\res \gets \res \cup \{ \breg \}$\;

            % Case (ii C)
        %    \If{$q_{\reg} \ge 1$}{
        %       $\breg_1 \gets$ copy of $\reg$\;
               % Possiamo già calcolare il caso (iii C) 
        %       \texttt{insert-and-remove-set}$(\breg_1, -q_{\breg_1}, 0)$\;
        %       $\breg_2 \gets$ copy of $\breg_1$\;
        %       \texttt{insert-and-remove-set}$(\breg_2, 1, 0)$\;
        %       $\res \gets \res \cup \{ \breg_1, \breg_2 \}$\;
        %    }
        %}    
        \Return $\res$\;
    }
\end{algorithm}



\begin{algorithm}[t]
    \caption{\texttt{delay-predecessors-A-C}$(\reg)$}
    
    \KwData{$\reg$: a region of either class A or class C.}
    \KwResult{The delay predecessors of $\reg$.}
    
    \Begin() {    
        $\breg \gets$ copy of $\reg$\;
        create empty set $X_{\mathit{tmp}}$\;
        \ForEach{$x \in X_{\breg,0}$}{
            $h_{\breg}(x) \gets h_{\breg}(x) - 1$\;
            $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{ x \}$\;
            $X_{\breg,0} \gets X_{\breg,0} \setminus x$\;
        }
        \texttt{insert-right}$(\breg, X_{\mathit{tmp}}, p_{\breg})$\;
        \Return $\{ \breg \}$\;
    }
\end{algorithm}
%\todoAM{}{Nell'algoritmo A e C, mettere $p_{\breg}$ va bene perchè se R è ri classe A allora p è 0, altrimenti p è maggiore di 0 e i clock vengono inseriti in fondo alla lista di quelli con parte frazionaria maggiore di 0.}
%
%
%
%
%%%%
%% ANDREBBERO INSERITI DEI SIDE CHECKS CHE CONTROLLANO CHE IL VALORE INTERO DEI CLOCK SIA MAGGIORE DI 0
%%%%
%% SE METTI H CAMBIA FONT METTENDOLO PIÙ GRANDE DI QUANDO USI tb
%%%%
%
% create empty set $X_{\mathit{tmp}}$\;
%                \texttt{insert-right}$(\reg, X_{\mathit{tmp}}, p_{\reg})$\;
%                
%                \For{$i = (p_{\reg} - 1)$ \KwTo $1$}{
%                    \ForEach{$x \in X_{\reg,i}$}{
%                        $X_{\reg,i+1} \gets X_{\reg,i+1} \cup \{x\}$\;
%                        $X_{\reg,i} \gets X_{\reg,i} \setminus \{x\}$\;
%                    }
%                }
%                
%                create empty set $X_{\mathit{oob}}$\;
%                \ForEach{$x \in X_{\reg,0}$}{
%                    \uIf{$h_{\reg}(x) = c_{\max}$}{
%                        $\mathit{X_{oob}} \gets \mathit{X_{oob}} \cup \{x\}$\;
%                    }
%                    \Else{
%                        $X_{\reg,1} \gets X_{\reg,1} \cup \{x\}$\;
%                    }
%                    $X_{\reg,0} \gets X_{\reg, 0} \setminus \{x\}$\;
%                }
%                
%                \If{$X_{\mathit{oob}} \neq \varnothing$}{
%                    \texttt{insert-left}$(\reg, X_{\mathit{oob}}, q_{\reg})$\;
%                }
%                
%                \If{$X_{\reg,1} = \varnothing$}{
%                    \texttt{remove}$(\reg, 1)$\;
%                }

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Delay_Predecessors/delay_predecessors.tex <==
\input{DelayAndDiscretePredecessors/Delay_Predecessors/find_delay_predecessors_algorithm}

\textbf{Immediate delay predecessors}~\Red{The following theorem (whose proof is shown in the Appendix, \autoref{thm:proof_of_bounded_d_pred}) establishes that, when tracking the order in which clocks become unbounded, the number of immediate delay predecessors of a given region does not exhibit exponential blow-up.}
%\todoAM{}{Per giustificare il teorema occorre dire che questo si applica quando ti va backwards da una regione unbounded? Se non si conoscesse l'ordine con cui i clock sono andati out of bounds, occorrerebbe provare tutte le combinazioni di predecessori.}

\begin{theorem}
\label{thm:bounded_d_pred}
   If the order in which clocks become unbounded is tracked, the number of immediate delay predecessors of a given region is at most three.
\end{theorem}

\Red{Indeed, if the order in which clocks become unbounded is not tracked, computing the immediate delay predecessors of regions with unbounded clocks would require enumerating all ordered partitions of the unbounded clocks, as every order in which the clocks become unbounded would then be admissible (regions without unbounded clocks would have a unique immediate delay predecessor).}

The immediate delay predecessors of a given region $\reg$ are computed by \autoref{alg:finddelaypred}, whose time complexity is $O(\lvert \ackc \rvert)$ (we refer to \emph{predecessors} in its description).
In particular, Line~\ref{line:dp:declarereg} initializes a set, returned in Line~\ref{line:dp:returnres}, storing the computed predecessors.
The algorithm proceeds by analyzing the class of $\reg$ to compute its predecessors by modifying a copy $\breg$ of $\reg$, created in Line~\ref{line:dp:copyr}.

If $\reg$ is of class $\cu$ (Line~\ref{line:dp:ucheck}), the predecessor is obtained by inserting set $X_{\breg, -\lidx_{\breg}}$, which contains the clocks that became unbounded while exiting from the unit, into $X_{\breg, 0}$.
Then, $X_{\breg, -\lidx_{\breg}}$ is removed from $\breg$ (Line~\ref{line:dp:handleuclass}).

For regions of class $\ca$ or class $\cc$ (Line~\ref{line:dp:accheck}),
an auxiliary set $X_{\mathit{tmp}}$ is initialized (Line~\ref{line:dp:initxtmp}).
The integer part of each clock $x \in X_{\breg, 0}$ (Line~\ref{line:dp:foreachloopac}) is decremented by 1 (Line~\ref{line:dp:decreaseh}), and $x$ is moved from $X_{\breg, 0}$ to $X_{\mathit{tmp}}$ (Line~\ref{line:dp:insertandremovex}). Since these clocks must have
the highest fractional part, $X_{\mathit{tmp}}$ is inserted to the right of $X_{\breg, \ridx_{\breg}}$ (Line~\ref{line:dp:insertxtmpright}).

If $\reg$ is of class $\cb$ (Line~\ref{line:dp:bcheck}), the algorithm considers both the cases where the predecessor is of class $\ca$ or class $\cc$. 
First, clocks in $X_{\breg, 1}$ (those that left the unit) are moved into $X_{\breg, 0}$ (Line~\ref{line:dp:insertx1inx0}). Then, Line~\ref{line:dp:checkunbound} checks whether unbounded clocks must also be handled.
If so, two additional regions are created.
The first, $\breg_1$, is created on Line~\ref{line:dp:copyinr1} as a copy of $\reg$ and updated on Line~\ref{line:dp:insertinr1} to represent the case in which all clocks with zero fractional part in the predecessor became unbounded.
After $\breg_1$ is updated, it is copied in $\breg_2$ (Line~\ref{line:dp:copyinr2}), which is modified on Line~\ref{line:dp:insertinr2} to capture the case in which only a subset of those clocks became unbounded.
Both $\breg_1$ and $\breg_2$ are collected on Line~\ref{line:dp:collectr1r2} in the result set.
%\todoMR{}{Quindi alla fine vengono restituite $\breg$, $\breg_1$ e $\breg_2$, perché comunque $\breg$ viene aggiunta alla fine; di fatto, $\breg$ è quella in cui solo i clock di $X_1$ tornano indietro, $\breg_1$ è quella in cui tornano indietro solo i clock di $X_{-\ell}$, e $\breg_2$ è quella in cui tornano entrambi indietro.}

%Given a region $\reg$ of a \ac{ta} $\aut$, \autoref{alg:finddelaypred} computes each immediate delay predecessor in at most $\lvert \ackc \rvert$ steps. 
%This follows by analyzing all branches of the conditional statements at lines \ref{line:dp:ucheck}, \ref{line:dp:accheck}, and \ref{line:dp:bcheck}.  
%By \autoref{thm:bounded_d_pred}, it follows that the computation of immediate delay predecessors of $\reg$ has time complexity $O(\lvert \ackc \rvert)$.


\input{DelayAndDiscretePredecessors/Figures/delaypredexamplecropped}

\begin{example}
\label{ex:delaypred}
Let $\aut$ be a \ac{ta} having clocks $\ackc = \{ x, y \}$ and maximum constant $\cmax = 2$.  
Consider the region $\reg_0$ 
%(for some location $q \in Q$), 
as depicted in \autoref{fig:partcompfig}.
Here, triangles are used to symbolically represent entire regions rather than individual points (\emph{e.g.}, the triangle
corresponding to $\reg_2$ represents the region 
$\{ (x, y) \; | \; 1 < x < 2 \land y > 2 \}$).
For this reason, they are not drawn on the diagonals, as would be implied by \autoref{def:clock_equivalence}.
\Red{For visual clarity, the figure does not represent the portion of the state space where $y < 1$.}
Since $\reg_0$ lies above the diagonal originating from $(2,2)$, it corresponds to the case in which $y$ became unbounded before $x$.  
$\reg_0$ can be represented as:
$
\mathcal{R}_0 = \{ q,\, h(x) = 2,\, h(y) = 2,\, X_{-2} = \{ x \},\, X_{-1} = \{ y \},\, X_0 = \varnothing \}.
$

We compute the delay predecessors of $\reg_0$ using \autoref{alg:finddelaypred}.  
For conciseness, we stop the computation when reaching a bounded region or because no further delay predecessors exist.  
The algorithm yields a single immediate delay predecessor of class $\ca$ (\autoref{fig:partcomptab}):
$
\mathcal{R}_1 = \{ q,\, h(x) = 2,\, h(y) = 2,\, X_{-1} = \{ y \},\, X_0 = \{ x \} \}
$.
%
Applying the same algorithm to $\reg_1$ yields a single immediate delay predecessor:
$
\mathcal{R}_2 = \{ q,\, h(x) = 1,\, h(y) = 2,\, X_{-1} = \{ y \},\, X_0 = \varnothing,\, X_1 = \{ x \} \}.
$
Then, from $\reg_2$, three immediate delay predecessors can be computed. Two of them ($\reg_4$ and $\reg_5$) are not further analyzed in this example, as they are already bounded.
%
Consider the region:
$
\mathcal{R}_3 = \{ q,\, h(x) = 1,\, h(y) = 2,\, X_{-1} = \{ y \},\, X_0 = \{ x \} \}.
$  
This region is structurally equivalent to $\reg_1$, except that the integer value of $x$ has been decremented by 1.
The computation from $\reg_1$ applies similarly from $\reg_3$.
%\todoAM{}{Forse si possono togliere le righe da computing the...}
%computing immediate delay predecessors until either:  
%(i) a bounded region is reached (though further exploration may still be possible), or  
%(ii) no delay predecessor exists, \emph{e.g.}, when a clock has an integer value equal to zero and no fractional part.
\end{example}

The computation of delay predecessors can be optimized.
Assume that, for a region $\reg$, \autoref{alg:finddelaypred} can be applied 
%an arbitrary number of 
$n$ times. 
Furthermore, assume that all clocks in $\reg$ are bounded and that $\ridx_{\reg} > 0$ holds.
%One can observe that, after $2 \cdot (\ridx_{\reg} + 1)$ iterations of \autoref{alg:finddelaypred} (if $X_{\reg, 0} \neq \varnothing$), or $2 \cdot \ridx_{\reg}$ iterations (if $X_{\reg, 0} = \varnothing$), the resulting region $\reg'$ is structurally equivalent to $\reg$, differing only in the integer values of clocks, each of which has been decreased by 1.
%
%Consider the region
%$\reg = \{q, h(x) = 2, h(y) = 3, h(z) = 2, X_0, X_1, X_2 \}$, where $X_{\reg,0} = \varnothing$, $X_{\reg,1} = \{ x \}$, and $X_{\reg,2} = \{ y, z \}$.
%Applying \autoref{alg:finddelaypred} four times to $\reg$ gives
%$\reg' = \{q, h(x) = 1, h(y) = 2, h(z) = 1, X_0 , X_1, X_2 \}$,
%where $X_{\reg',0} = \varnothing$, $X_{\reg',1} = \{ x \}$, and $X_{\reg',2} = \{ y, z \}$ capture the same clock partitioning as in $\reg$.
%
%This reasoning, for regions in which all clocks are bounded, can be generalized as follows.  
%Suppose we want to apply \autoref{alg:finddelaypred} $n$ times to a given region $\reg$. 
We define the \emph{period} of $\reg$ as
$\theta = 2 \cdot (\ridx_{\reg} + 1)$ if $X_{\reg, 0} \neq \varnothing$; $\theta = 2 \cdot \ridx_{\reg}$ otherwise.
Then, decrement the integer value of every clock of $\reg$ by $\lfloor n / \theta \rfloor$ (ensuring their integer value does not go below zero), obtaining a new region $\reg'$.
After this step, if none of the clocks of $\reg'$ are equal to zero \Red{(with no fractional part)}, it suffices to apply \autoref{alg:finddelaypred} only $n \bmod \theta$ times to $\reg'$ to obtain the final result, possibly stopping earlier if one or more clocks become equal to zero during this process.
Similar optimizations can also be applied when some clocks are unbounded.  
%For example, if a subset of clocks remains always unbounded (this can happen as illustrated intuitively in \autoref{fig:partcompfig}), the approach described above can be applied analogously by considering only the bounded clocks.

%When at least one clock in a region is exactly equal to zero, delay predecessors cannot be computed, as clock values cannot be negative. 
%In such cases, however, discrete predecessors may still be computed.

\textbf{Discrete predecessors (intuition)}~When computing a discrete successor, a subset of clocks may be reset, and therefore appear with value zero in the successor region. 
Discrete predecessors computation aims to reverse this operation. 
However, starting from a region in which the value of some clocks is zero (with no fractional part), a challenge arises, since the original values of these clocks prior to being reset are unknown. 
As a result, all possible combinations of values for the reset clocks must be considered (including cases where they may have been unbounded) to ensure all discrete predecessors are computed.
This process can be simplified using the guard of the transition over which discrete predecessors are computed, as it may constrain the possible values of clocks prior to reset.

The following theorem (whose proof is shown in the Appendix, \autoref{thm:proof_of_discrete_predecessor_complexity}) establishes that, when tracking the order in which clocks become unbounded, the number of discrete predecessors of a given region suffers from an inherent exponential blow-up that cannot be avoided in general.
%\todoAM{}{Nello statement del teorema 2, tenere 'must be tracked' o mettere 'is known'?}

\begin{theorem}
\label{thr:discrete_predecessor_complexity}
    Let $\aut$ be a \ac{ta} such that $n = \lvert \ackc \rvert$ and let $\reg$ be a region of $\aut$. If the order in which clocks become unbounded must be tracked, then the number of discrete predecessors of $\reg$ over a single transition is $O\left( (\frac{\cmax + 1}{\ln 2}) ^{n}\cdot (n+1)!\right)$.
\end{theorem}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Delay_Predecessors/find_delay_predecessors_algorithm.tex <==
\begin{algorithm}[t]
    \caption{\texttt{find-immediate-delay-predecessors}$(\reg)$}
    \label{alg:finddelaypred}
    
    \KwData{$\reg$: a region where no clock $x$ is such that: $h_{\reg}(x) = 0 \land x \in X_{\reg, 0}$.}
    \KwResult{The immediate delay predecessors of $\reg$.}
    \Begin() {
        %\tcp{We assume no clock $x$ is such that $h(x) = 0 \land x \in X_0$}
        $\res \gets \varnothing$\; \label{line:dp:declarereg}
        $\breg \gets$ copy of $\reg$\; \label{line:dp:copyr}
        \uIf{$X_{\reg,0} = \varnothing \land \ridx_{\reg} = 0$}{ \label{line:dp:ucheck}
            %\tcp{$\reg$ belongs to class U}
            %$\breg \gets$ copy of $\reg$\;
            insert clocks of $X_{\breg, -\lidx_{\breg}}$ in $X_{\breg, 0}$ and remove $X_{\breg, -\lidx_{\breg}}$ from $\breg$\;
            \label{line:dp:handleuclass}
            %\texttt{insert-and-remove-set}$(\breg, -\lidx_{\breg}, 0)$\;
            %$\res \gets \res \cup \{ \breg \}$\;
        }
        \uElseIf{$X_{\reg,0} \neq \varnothing$}{ \label{line:dp:accheck}
            %\tcp{$\reg$ belongs to either class A or class C}
            %$\breg \gets$ copy of $\reg$\;
            $X_{\mathit{tmp}} \gets \varnothing$\; \label{line:dp:initxtmp}
            \ForEach{$x \in X_{\breg,0}$}{ \label{line:dp:foreachloopac}
                $h_{\breg}(x) \gets h_{\breg}(x) - 1$\; \label{line:dp:decreaseh}
                $X_{\mathit{tmp}} \gets X_{\mathit{tmp}} \cup \{ x \}$; 
                $X_{\breg,0} \gets X_{\breg,0} \setminus \{ x \}$\; \label{line:dp:insertandremovex}
            }
            insert $X_{\mathit{tmp}}$ to the right of $X_{\breg, \ridx_{\breg}}$\; \label{line:dp:insertxtmpright}
            %\texttt{insert-right}$(\breg, X_{\mathit{tmp}}, \ridx_{\breg})$\;
            %$\res \gets \res \cup \{ \breg \}$\;
        }
        %\ElseIf{$\ridx_{\reg} > 0 \land X_{\reg,0} = \varnothing$}{ 
        \Else{
        \label{line:dp:bcheck}
            %\tcp{$\reg$ belongs to class B}
            %$\breg \gets$ copy of $\reg$\;
            insert clocks of $X_{\breg, 1}$ in $X_{\breg, 0}$ and remove $X_{\breg, 1}$ from $\breg$\; \label{line:dp:insertx1inx0}
            %\texttt{insert-and-remove-set}$(\breg, 1, 0)$\;
            %$\res \gets \res \cup \{ \breg \}$\;

            \If{$\lidx_{\reg} \ge 1$}{ \label{line:dp:checkunbound}
                $\breg_1 \gets$ copy of $\reg$\; \label{line:dp:copyinr1}
                insert clocks of $X_{\breg_1, -\lidx_{\breg_1}}$ in $X_{\breg_1, 0}$ and remove $X_{\breg_1, -\lidx_{\breg_1}}$ from $\breg_1$\; \label{line:dp:insertinr1}
                %\texttt{insert-and-remove-set}$(\breg_1, -\lidx_{\breg_1}, 0)$\;
                $\breg_2 \gets$ copy of $\breg_1$\; \label{line:dp:copyinr2}
                insert clocks of $X_{\breg_2, 1}$ into $X_{\breg_2, 0}$ and remove $X_{\breg_2, 1}$ from $\breg_2$\; \label{line:dp:insertinr2}
                %\texttt{insert-and-remove-set}$(\breg_2, 1, 0)$\;
                $\res \gets \res \cup \{ \breg_1, \breg_2 \}$\; \label{line:dp:collectr1r2}
             }
        }
        %$\res \gets \res \cup \{ \breg \}$\;
        \Return ($\res \cup \{ \breg \})$\; \label{line:dp:returnres}
    }
\end{algorithm}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Discrete_Predecessors/backups/discrete_predecessors_algorithm_backup.tex <==
\begin{algorithm}[tb]
    \caption{\texttt{find-discrete-predecessors}$(\reg)$}

    
    \KwData{$\reg$: a region.}
    \KwResult{The set of regions reachable via backward discrete transitions from $\reg$.}
    
    \Begin(){
        $\mathit{res} \gets \varnothing$\;
        
        %\tcp{Get discrete transitions in the original \ac{ta} ending in $\mathit{loc}_{\reg}$}
        $\mathcal{T} \gets \{ (\mathit{loc}', a, \gamma, Y, \mathit{loc}_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, \mathit{loc}' \in Q \}$\;

        \ForEach{$t \in \mathcal{T}$}{
        
        $X_{\mathit{bnd}} \gets \varnothing$\;
        $X_{\mathit{oob}} \gets \varnothing$\;
        
        \ForEach{clock constraint $\ccstr \in \gamma$}{
            $\breg \gets$ copy of $\reg$\;

            \uIf{$(\ccstr{}$ is an equality constraint: $x = c) \land (x \in Y)$}{
                $h_{\breg}(x) = c$\;
            }

            \uElseIf{$(\ccstr{}$ is an inequality constraint: $x > \cmax) \land (x \in Y)$}{
                $X_{\mathit{oob}} \gets X_{\mathit{oob}} \cup \{ x \}$\;
            }

            \ElseIf{$x \in Y$}{
                $X_{\mathit{bnd}} \gets X_{\mathit{bnd}} \cup \{ x \}$\;
            }
        }

        $\mathit{tmp} \gets \varnothing$\;
        $\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
        $\Pi_{\mathit{oob}} \gets $ all partitions of $X_{\mathit{oob}}$\;

        \ForEach{partition $\pi \in \Pi_{\mathit{oob}}$}{
            %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
            $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
            \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                $\mathit{tmp} \gets \mathit{tmp} \cup \{ \breg' \}$\;
            }
        }

        \ForEach{$\mathcal{H} \in \{0, 1, \dots, \cmax + 1\}^{\lvert X_{\mathit{bnd}} \rvert}$}{
            \If{each $x \in X_{\mathit{bnd}}$ can have $h(x)$ according to $\mathcal{H}$ and $\gamma$}{
                $\mathit{tmp}' \gets$ copy of $\mathit{tmp}$\;
                
                \If{some clocks $\Delta \subseteq X_{\mathit{bnd}}$ are unbounded}{

                    \ForEach{$\breg \in \mathit{tmp}$}{

                    $\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
                    $\Pi_{\Delta} \gets $ all partitions of $X_{\Delta}$\;

                    \ForEach{partition $\pi \in \Pi_{\Delta}$}{
                        $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                        \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                            $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                            $\mathit{tmp}' \gets \mathit{tmp}' \cup \{ \breg' \}$\;
                        }
                    }
                    }
                }

                \ForEach{$\breg \in \mathit{tmp}'$}{
                    $\mathcal{X} \gets \{ X_{\breg, 1}, \dots, X_{\breg, p_{\breg}} \}$\;
                    $\Pi_{\mathit{bnd}} \gets $ all partitions of $X_{\mathit{bnd}}$\;

                    \ForEach{partition $\pi \in \Pi_{\mathit{bnd}}$}{
                        $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                       %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                        \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                            $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $o$ and where clocks have an integer value according to $\mathcal{H}$\;
                            $\res \gets \res \cup \{ \breg' \}$\;
                        }
                    }
                }
                
            }
        }
        }

        \Return $\res$\;
    }
\end{algorithm}

\todoAM{}{vedere se tenere questa notazione ed eventualmente adattare il resto prima}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Discrete_Predecessors/backups/discrete_predecessors_v2.tex <==
\begin{algorithm}[!hb]
    \caption{\texttt{find-discrete-predecessors}$(\reg)$}

    
    \KwData{$\reg$: a region.}
    \KwResult{The set of regions reachable via backward discrete transitions from $\reg$.}
    
    \Begin(){
        $\mathit{res} \gets \varnothing$\;
        
        %\tcp{Get discrete transitions in the original \ac{ta} ending in $\mathit{loc}_{\reg}$}
        %$\mathcal{T} \gets \{ (\mathit{loc}, a, \gamma, Y, \mathit{loc}_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, \mathit{loc} \in Q \}$\;

        \ForEach{$t \in \{ (q, a, \gamma, Y, q_{\reg}) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, q \in Q \}$}{
        
        $X_{\mathit{bnd}} \gets \varnothing$; $X_{\mathit{oob}} \gets \varnothing$\;
        $\breg \gets$ copy of $\reg$\;
        
        \ForEach{clock constraint $\ccstr \in \gamma$}{

            \uIf{$(\ccstr{}$ is an equality constraint: $x = c) \land (x \in Y)$}{
                $h_{\breg}(x) = c$\;
            }

            \uElseIf{$(\ccstr{}$ is an inequality constraint: $x > \cmax) \land (x \in Y)$}{
                $X_{\mathit{oob}} \gets X_{\mathit{oob}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\;
            }

            \ElseIf{$($clock $x$ appears in $\ccstr) \land (x \in Y)$}{
                $X_{\mathit{bnd}} \gets X_{\mathit{bnd}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\;
            }
        }
        
        %$\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
        %$\Pi_{\mathit{oob}} \gets $ all partitions of $X_{\mathit{oob}}$\;

        %\ForEach{partition $\pi \in \Pi_{\mathit{oob}}$}{
        %    %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
        %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
        %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
        %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
        %        $\mathit{tmp} \gets \mathit{tmp} \cup \{ \breg' \}$\;
        %    }
        %}

        $\mathit{tmp} \gets$ \texttt{perm-regs}($\breg, -q_{\breg}, -1, X_\mathit{oob}, h_{\breg}, \varnothing$)\;

        \ForEach{$h \in \{0, 1, \dots, \cmax + 1\}^{\lvert X_{\mathit{bnd}} \rvert}$}{
            \If{$\forall x \in X_{\mathit{bnd}} : h(x) = h_{\breg}(x)$ and $h$ satisfies $\gamma$}{
                $\mathit{tmp}' \gets$ copy of $\mathit{tmp}$\;
                $\Delta \gets \{ x \in X_{\mathit{bnd}} \; \vert \; h(x) > \cmax \}$\;
                
                \If{$\Delta \neq \varnothing$}{

                    \ForEach{$R \in \mathit{tmp}$}{

                    %$\mathcal{X} \gets \{ X_{\breg, -q_{\breg}}, \dots, X_{\breg, -1} \}$\;
                    %$\Pi_{\Delta} \gets $ all partitions of $X_{\Delta}$\;

                    %\ForEach{partition $\pi \in \Pi_{\Delta}$}{
                    %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                    %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                    %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $\zeta$\;
                    %        $\mathit{tmp}' \gets \mathit{tmp}' \cup \{ \breg' \}$\;
                    %    }
                    $\mathit{tmp}' \gets \mathit{tmp}'$ $\cup$ \texttt{perm-regs}($R, -q_R, -1, \Delta, h_R, X_{\mathit{oob}}$)\;
                    }
                }

                \ForEach{$R \in \mathit{tmp}'$}{
                    %$\mathcal{X} \gets \{ X_{\breg, 1}, \dots, X_{\breg, p_{\breg}} \}$\;
                    %$\Pi_{\mathit{bnd}} \gets $ all partitions of $X_{\mathit{bnd}}$\;

                    %\ForEach{partition $\pi \in \Pi_{\mathit{bnd}}$}{
                    %    $\mathcal{Z} \gets$ all permutations of $\mathcal{X} \cup \pi$ that preserve the order of $\mathcal{X}$\;
                       %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                    %    \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                    %        $\breg' \gets $ copy of $\breg$ with sets $\mathcal{X} \cup \pi$ reordered according to $o$ and where clocks have an integer value according to $\mathcal{H}$\;
                    %        $\res \gets \res \cup \{ \breg' \}$\;
                    %    }
                    $\res \gets \res$ $\cup$ \texttt{perm-regs}($R, 1, p_R, X_{\mathit{bnd}} \setminus \Delta, h, \varnothing$)\;
                    }
            }

        }
                
        }

        \Return $\res$\;

        \BlankLine
        \BlankLine

        \SetKwFunction{gaop}{perm-regs}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\gaop{$\reg, i, j, X, \mathcal{H}, X_{\mathit{ignore}}$}}{
            $\res \gets \varnothing$\;
            clamp to $\cmax$ all values of $\mathcal{H}$ that are greater than $\cmax$\;
            $\mathcal{X} \gets \{ X_{\reg, i}, \dots, X_{\reg, j} \} \setminus X_{\mathit{ignore}}$\;
            $\Pi \gets $ all partitions of $X$\;

            \ForEach{partition $\pi \in \Pi$}{
                $\mathcal{Z} \gets$ all permutations of ($\mathcal{X} \cup \pi$) that preserve the order of $\mathcal{X}$\;
                %\tcp{Generate permutations of $\mathcal{X} \cup \pi$ preserving the order of $\mathcal{X}$}
                \ForEach{permutation $\zeta \in \mathcal{Z}$}{
                   $\breg \gets $ copy of $\reg$ such that (i) sets ($\mathcal{X} \cup \pi$) are reordered according to $\zeta$ and (ii) clocks have a value given by $\mathcal{H}$\;
                   $\res \gets \res \cup \{ \breg \}$\;
                }
           }
           \Return $\res$\;
        }        
    }
\end{algorithm}

\todoAM{}{Cambiare in tutto il paper l'indice $q$ con $\ell$ e $p$ con $r$ OKKIO anche al teorema 2}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Discrete_Predecessors/discrete_predecessor_algorithm.tex <==
\begin{algorithm}[t]
    \caption{\texttt{find-discrete-predecessors}$(\reg)$}
    \label{alg:finddiscretepred}
    
    \KwData{$\reg$: a region.}
    \KwResult{The discrete predecessors of $\reg$.}
    
    \Begin(){
        $\mathit{res} \gets \varnothing$\; \label{line:fdp:resempty}
        
        \ForEach{$t  = (q, a, \gamma, Y, q_{\reg})  \in  T$}{ \label{line:fdp:startloop}
        
        $X_{\mathit{bnd}} \gets \varnothing$; $X_{\mathit{oob}} \gets \varnothing$\; \label{line:fdp:initbndoob}
        $\breg \gets$ copy of $\reg$\; \label{line:fdp:copyr}
        $\allclocks{\breg} \gets$ a reference to the clocks of $\breg$\; \label{line:fdp:clockreference}
        $q_{\breg} \gets q$\; \label{line:fdp:assignq}

        \ForEach{clock $x \in Y$} { \label{line:fdp:foreachcconstr}

            \uIf{$x$ belongs to a constraint of the form $(x = c) \in \gamma$}{ \label{line:fdp:isequality1}
                $h_{\breg}(x) = c$\; \label{line:fdp:isequality2}
            }

            \uElseIf{$x$ belongs to a constraint of the form $(x > \cmax) \in \gamma$}{ \label{line:fdp:isunbo1}
                $h_{\breg}(x) = \cmax$\; \label{line:fdp:assignqoob}
                $X_{\mathit{oob}} \gets X_{\mathit{oob}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\; \label{line:fdp:isunbo2}
            }

            \Else{ \label{line:fdp:isbound1}
                $X_{\mathit{bnd}} \gets X_{\mathit{bnd}} \cup \{ x \}$;
                $\allclocks{\breg} \gets \allclocks{\breg} \setminus \{ x \}$\;  \label{line:fdp:isbound2}
            }
        }

        \uIf{$X_{\mathit{bnd}} = \varnothing$}{ \label{line:fdp:bndisempty}
            $\res \gets \res$ $\cup$ \texttt{part-regs}($\breg, -\lidx_{\breg}, -1, X_\mathit{oob}, h_{\breg}$)\; \label{line:fdp:oobfubini}
        }
        \Else{

        \ForEach{function $\bar{h} : X_{\mathit{bnd}} \to \{0, \dots, \cmax + 1\}$}{ \label{line:fdp:foreachfunc}
           
            %\If{$\gamma$ is satisfied by $\bar{h}$, $h_{\breg}$, and the clocks in $X_\mathit{oob}$}{
            \label{line:fdp:gammasatisfiedbyh}
                
                $\Delta \gets \{ x \in X_{\mathit{bnd}} \; \vert \; \bar{h}(x) > \cmax \}$\; \label{line:fdp:createdelta}
                
                \ForEach{$R \in$ \textnormal{\texttt{part-regs}}$(\breg, -\lidx_{\breg}, -1, X_\mathit{oob} \cup \Delta, \bar{h} \cup h_{\breg})$}{ \label{line:fdp:allrinpermreg}
                    $\res \gets \res$ $\cup$ \texttt{part-regs}($R, 0, \ridx_R, X_{\mathit{bnd}} \setminus \Delta, \bar{h} \cup h_{R}$)\; \label{line:fdp:resUres}
                    }
            }
        }   
        %}
        remove from $\res$ all regions not satisfying $\gamma$\; \label{line:fdp:removefromres}
        }

        \Return $\res$\; \label{line:fdp:returnres}
}
\end{algorithm}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Discrete_Predecessors/discrete_predecessors.tex <==
\input{DelayAndDiscretePredecessors/Discrete_Predecessors/discrete_predecessor_algorithm}

\begin{algorithm}[th]
    \caption{\texttt{part-regs}$(\reg, i, j, X, \mathcal{H})$}
    \label{alg:perm-regs}
    
    \KwData{$\reg$: a region; 
    $i, j$: two integers such that $i \le j$ holds;
    $X$: a set of clocks,
    $\mathcal{H}$: a function assigning integer values to clocks.}
    \KwResult{all regions obtained from $\reg$ by finding all ordered partitions of $X$ while preserving the relative order of $X_{\reg,i}, \dots, X_{\reg,j}$.}
    \Begin(){
            $\res \gets \varnothing$\; \label{line:fdppr:res}
            $\breg \gets $ copy of $\reg$\; \label{line:fdppr:copyreg}

            \If{$X = \varnothing$}{ \label{line:fdppr:xisempty}
                \Return $\{ \reg \}$\; \label{line:fdppr:returnbregxempty}
            }

            \ForEach{$x \in X$}{ \label{line:fdppr:foreachx}
                \If{$i \ge 0 \land \mathcal{H}(x) = \cmax$}{ \label{line:fdppr:iandhxcond}
                    $X_{\breg, 0} \gets X_{\breg, 0} \cup \{ x \}$;
                    $X \gets X \setminus \{ x \}$\; \label{line:fdppr:removeinsertx}
                }
            }
            $\mathcal{X} \gets \{ X_{\breg, i}, \dots, X_{\breg, j} \}$\; \label{line:fdppr:preserve}
            $\Pi \gets $ all partitions of $X$\; \label{line:fdppr:partitions}

            \ForEach{partition $\pi \in \Pi$}{ \label{line:fdppr:forpartitions}
                \begin{varwidth}[t]{0.8\linewidth}{$\mathcal{Z} \gets$ ordered partitions of $(\mathcal{X} \cup \pi)$ that preserve the relative order of the elements in $\mathcal{X}$; these partitions are obtained by computing all permutations of $\pi$ and interleaving them with $\mathcal{X}$, allowing elements of $\pi$ to also be inserted within the elements of $\mathcal{X}$}\; \label{line:fdppr:orderedpartitions}
                \end{varwidth}
                \nl
                \ForEach{ordered partition $\zeta \in \mathcal{Z}$}{ \label{line:fdppr:foreachpermut}
                   \begin{varwidth}[t]{0.8\linewidth}{$R \gets $ copy of $\breg$ such that ($\mathcal{X} \cup \pi$) are partitioned according to $\zeta$ and clocks have a value given by $\mathcal{H}$ (if $\mathcal{H}(x) > \cmax$, then assign $\cmax$ to $x$)\;} \label{line:fdppr:computecopy}
                   \end{varwidth}
                   \nl
                   $\res \gets \res \cup \{ R \}$\; \label{line:fdppr:collectr}
                }
           }
           \Return $\res$\; \label{line:fdppr:returnres}
        }        
\end{algorithm}

The discrete predecessors of a region $\reg$ can be computed using \autoref{alg:finddiscretepred}.
In particular, Line~\ref{line:fdp:resempty} initializes a set storing the computed predecessor regions.
A loop over all transitions $t$ ending in $q_{\reg}$, the location of $\reg$, 
begins at Line~\ref{line:fdp:startloop}.
Line~\ref{line:fdp:initbndoob} initializes a set $X_{\mathit{bnd}}$, which will contain clocks
that were bounded or possibly unbounded, and a set $X_{\mathit{oob}}$, which will contain clocks that were certainly unbounded (in a predecessor).
A copy $\breg$ of $\reg$ is made at Line~\ref{line:fdp:copyr}.
Line~\ref{line:fdp:clockreference} creates a reference $\allclocks{\breg}$ to the clock sets of $\breg$, meaning that changes to $\allclocks{\breg}$ (\emph{e.g.}, removing a clock) directly affect $\breg$.
The location of $\breg$ is updated on Line~\ref{line:fdp:assignq} to match the one where $t$ originates.
%\Red{The loop at Line~\ref{line:fdp:foreachcconstr} examines each clock constraint $\xi$ appearing in the guard %$\gamma$ of $t$ and considers each clock $x$ only if it appears in $\xi$ and it is reset:
%(i) if $\xi$ is an equality, only the value of $x$ must be set (Lines~\ref{line:fdp:isequality1}--%\ref{line:fdp:isequality2});
%(ii) if $x$ was unbounded, $x$ is added to $X_{\mathit{oob}}$ and removed from $\reg$ (Lines~\ref{line:fdp:isunbo1}--%\ref{line:fdp:isunbo2}), while its integer value is set to $\cmax$ (Line~\ref{line:fdp:assignqoob});
%(iii) otherwise, $x$ was bounded or possibly unbounded, hence
%$x$ is added to $X_{\mathit{bnd}}$ and removed from $\reg$ (Lines~\ref{line:fdp:isbound1}--\ref{line:fdp:isbound2}).}
\Red{Then, the loop at Line~\ref{line:fdp:foreachcconstr} examines each reset clock $x \in Y$:
(i) if $x$ appears in an equality clock constraint of the form $(x = c) \in \gamma$, only the integer value of $x$ must be set (Lines~\ref{line:fdp:isequality1},\ref{line:fdp:isequality2});
(ii) if $x$ was unbounded, \emph{i.e.}, it appears in an inequality constraint of the form $(x > \cmax) \in \gamma$, $x$ is added to $X_{\mathit{oob}}$ and removed from $\breg$ (Lines~\ref{line:fdp:isunbo1},\ref{line:fdp:isunbo2}), while its integer value is set to $\cmax$ (Line~\ref{line:fdp:assignqoob});
(iii) otherwise, $x$ was bounded or possibly unbounded, hence
$x$ is added to $X_{\mathit{bnd}}$ and removed from $\breg$ (Lines~\ref{line:fdp:isbound1},\ref{line:fdp:isbound2}).
The latter case also accounts for reset clocks $x' \in Y$ that do not appear in any constraint of $\gamma$, which is equivalent to assuming a trivial constraint of the form $(x' \geq 0) \in \gamma$.
It is important to note that every clock in $Y$ is required to be exactly zero, \emph{i.e.}, to have an integer value equal to zero and no fractional part, since all clocks in $Y$ are reset along transition $t$.}

If $X_{\mathit{bnd}}$ is empty (Line~\ref{line:fdp:bndisempty}), the predecessors over the current transition are computed by finding all ordered partitions of $X_{\mathit{oob}}$, preserving the order of unreset unbounded clocks. This is performed at Line~\ref{line:fdp:oobfubini} using the auxiliary algorithm \emph{part-regs}$(\reg', i, j, X, \mathcal{H})$,
which computes all regions derived from the input region $\reg'$ by finding all ordered partitions of a clock set $X$, while preserving the order of \Red{clock sets} $X_{\reg',i}, \dots, X_{\reg',j}$ (where $i \leq j$).
For each resulting region, the integer value of every clock $x$ is given by $\mathcal{H}(x)$.
\Red{If $X = \varnothing$, \emph{part-regs} returns the input region $\reg'$ unchanged.  
This also covers the case where a transition does not reset any clock; in such a situation, both $X_{\mathit{bnd}}$ and $X_{\mathit{oob}}$ are empty, and Line~\ref{line:fdp:oobfubini} simply inserts $\breg$ into the result set.}
The pseudocode of \emph{part-regs} is given in \autoref{alg:perm-regs}, and a detailed description follows at the end of this section.

Otherwise, all combinations of integer values (and potential unboundedness) for clocks in $X_{\mathit{bnd}}$ must be considered. This is done in the loop at Line~\ref{line:fdp:foreachfunc}, which iterates over all functions $\bar{h}$ defined on $X_{\mathit{bnd}}$. Note that $\bar{h}$ maps only clocks in $X_{\mathit{bnd}}$, while $h_{\breg}$ maps clocks in $\allclocks{\breg} \setminus X_{\mathit{bnd}}$; the conventional value $\cmax + 1$ captures the case in which a clock was unbounded in the predecessor.
%\Red{On Line~\ref{line:fdp:gammasatisfiedbyh}, we check whether $\gamma$ is satisfied by $\bar{h}$, $h_{\breg}$, and the clocks in $X_{\mathit{oob}}$. 
%This is done by combining the integer values of the clocks, as given by $\bar{h}$ and $h_{\breg}$, with their corresponding fractional parts. 
%For readability, a function assigning integer values to the clocks in $X_{\mathit{oob}}$ is not explicitly listed in the condition, since the value of these clocks is known to exceed $\cmax$.
%If the condition holds, then all clocks in $X_{\mathit{bnd}}$ that are unbounded under $\bar{h}$ (\emph{i.e.}, their integer value as returned by $\bar{h}$ is $\cmax$ + 1) are collected into a set $\Delta$ (Line~\ref{line:fdp:createdelta}).}
%If $\gamma$ is satisfied by $\bar{h}$ and $h_{\breg}$ (\emph{i.e.}, by combining the integer values of the clocks, as returned by $\bar{h}$ and $h_{\breg}$, with their fractional parts) (Line~\ref{line:fdp:gammasatisfiedbyh}), then 
All clocks in $X_{\mathit{bnd}}$ that are unbounded under $\bar{h}$ ({\emph{i.e.}, the integer value of these clocks returned by $\bar{h}$ is $\cmax$ + 1}) are collected into a set $\Delta$ (Line~\ref{line:fdp:createdelta}).
The loop at Line~\ref{line:fdp:allrinpermreg} iterates over all regions generated by \emph{part-regs} from $\breg$ partitioning $X_{\mathit{oob}} \cup \Delta$, preserving the order of unreset unbounded clocks.
For each such region $R$, \emph{part-regs} is applied on Line~\ref{line:fdp:resUres} to $R$ partitioning $X_{\mathit{bnd}} \setminus \Delta$ (\emph{i.e.}, the bounded clocks), preserving the order of unreset bounded clocks.
\Red{On Line~\ref{line:fdp:removefromres}, all regions not satisfying the guard $\gamma$ of $t$ are removed from $\mathit{res}$.}
Line~\ref{line:fdp:returnres} returns the discrete predecessors of $\reg$.

\Red{It is worth noting that the total number of functions $\bar{h}$ defined over $X_{\mathit{bnd}}$ in Line~\ref{line:fdp:foreachfunc} can be reduced by tracking the minimum and maximum integer values that the clocks may assume. 
For example, consider two clocks $x,y$ appearing in the constraints $1 \leq x \land x \leq 4 \land y \geq 5$. 
In this case, it is unnecessary to generate all combinations of integer values for $x$ and $y$ from $0$ to $\cmax + 1$; instead, it suffices to generate combinations where $\bar{h}(x) \in [1,4]$ and $\bar{h}(y) \in [5,\cmax+1]$.
In addition, note that \emph{part-regs} may generate invalid regions that must be discarded. 
This occurs, for instance, when a clock $x$ appears in a constraint $x > c$ and is assigned the integer value $\bar{h}(x) = c$. 
In this case, $x$ must have a fractional part greater than zero; however, when computing all possible ordered partitions, it may happen that $x$ is assigned no fractional part. 
Similarly, if $x$ appears in a constraint $x \le c$ and is assigned $\bar{h}(x) = c$, it must have a fractional part equal to zero, but the computation of ordered partitions may assign it a fractional part greater than zero.  
These incorrect edge cases can be handled by adding additional checks to Algorithm~\ref{alg:finddiscretepred} and \emph{part-regs}, which are omitted here for conciseness.}
%It is easy to verify that, given a region $\reg$, \autoref{alg:finddiscretepred} exhibits such a combinatorial explosion.  
%Let $\mathit{DiPr}_{t}$ denote the total number of discrete predecessors of $\reg$ computed over a transition $t \in T$ of a given \ac{ta}, as characterized by \autoref{thr:discrete_predecessor_complexity}.  
%Let $\mathit{DiPr} = \sum_{t \in T} \mathit{DiPr}_{t}$ be the total number of discrete predecessors of $\reg$ across all transitions  
%$t = (q, a, \gamma, Y, q_{\reg}) \in T$ ending in $q_{\reg}$.  
%It follows that the time complexity of computing the discrete predecessors of $\reg$ is in $O(\mathit{DiPr})$.

\textbf{Description of \emph{part-regs}}~Line~\ref{line:fdppr:res} initializes the result set.
Then, a copy $\breg$ of $\reg$ is made on Line~\ref{line:fdppr:copyreg} to avoid modifying the original input region.
Notice that, if the set $X$ is empty (Line~\ref{line:fdppr:xisempty}), $X$ has exactly one partition, \emph{i.e.}, the empty set itself. 
Therefore, for convenience, the original region is returned on Line~\ref{line:fdppr:returnbregxempty}.
The loop at Line~\ref{line:fdppr:foreachx} processes each clock $x \in X$, checking if it can be inserted into $X_{\breg, 0}$ (Line~\ref{line:fdppr:iandhxcond}) and doing so at Line~\ref{line:fdppr:removeinsertx}, while also removing $x$ from $X$.
This is done since a bounded clock can have an integer value equal to $\cmax$ only when it has no fractional part.
Lines~\ref{line:fdppr:preserve} and \ref{line:fdppr:partitions} compute the sets for which the order must be preserved and the partitions $\Pi$ of $X$, respectively.

The loop at Line~\ref{line:fdppr:forpartitions} iterates over $\Pi$, generating ordered partitions preserving the order of $\mathcal{X}$ (\emph{e.g.}, in a valid ordered partition involving $\mathcal{X} = \{X_1, X_2, X_3\}$, $X_1$ appears before $X_2$, which appears before $X_3$).
Ordered partitions are computed at Line~\ref{line:fdppr:orderedpartitions}; some of them may involve inserting elements of a given partition $\pi \in \Pi$ into elements of $\mathcal{X}$.
For each valid ordered partition $\zeta$ (Line~\ref{line:fdppr:foreachpermut}), a region is created by copying $\breg$ (Line~\ref{line:fdppr:computecopy}), updating its sets of clocks according to $\zeta$, and using $\mathcal{H}$ for assigning integer values to clocks (the values returned by $\mathcal{H}$ are clamped to ensure no value exceeds $\cmax$).
Each such region is added to the result set (Line~\ref{line:fdppr:collectr}), which is returned on Line~\ref{line:fdppr:returnres}.

\begin{example}
    Let $\aut$ be a \ac{ta} such that $\ackc = \{ x, y, w, p, z, s \}$ and $\cmax = 5$, and let $t = (q_0, a, \gamma, Y, q) \in T$, where $\gamma :=x \ge 0 \land y \ge 1 \land  w > 5 \land p = 1 \land z > 3 \land s > 4$ and $Y = \{ x, y, w, p \}$, be the transition of $\aut$ over which, for illustrative purposes, we compute only one discrete predecessor, which we refer to as $\breg$, of the following region:
    $
    \reg = \{ q, h(x) = h(y) = h(w) = h(p) = 0, h(z) = h(s) = 4, X_0, X_1, X_2 \}
    $,
    where $X_0 = \{x, y, w, p \}$, $X_1 = \{ z \}$, and $ X_2 = \{ s \}$.
    To better understand how \autoref{alg:finddiscretepred} works, we reference some of its lines in the following computation.

    Since clocks $z$ and $s$ are not reset in $t$, they do not influence the computation of $\breg$.  
    From the analysis of $Y$ (Lines~\ref{line:fdp:foreachcconstr} through~\ref{line:fdp:isbound2}), we can infer the following: $x$ and $y$ may have been either bounded or unbounded in $\breg$ (here, we assume they were bounded), $w$ was unbounded, and $p$ had the value $1$ with no fractional part.
    In particular, $x$ and $y$ are now collected in $X_{\mathit{bnd}}$.
    %
    Since $x$ and $y$ are assumed to be bounded in $\breg$, all possible combinations of their integer values must now be considered. 
    For the purposes of this example, a single combination suffices.
    Let $\bar{h}$ (Line~\ref{line:fdp:foreachfunc}) be such that $\bar{h}(x) = 3$ and $\bar{h}(y) = 2$ (this allows to satisfy $\gamma$ on Line~\ref{line:fdp:removefromres}, since $h_{\breg}(w) = 5$, $h_{\breg}(p) = 1$, and $h_{\breg}(z) = h_{\breg}(s) = 4$).
    %
    Since the order of the fractional parts of $x$ and $y$ in $\breg$ is unknown, all possible ordered partitions of $X_{\mathit{bnd}}$ and $X_{\mathit{oob}}$ must be explored, while preserving the order of the fractional parts of $z$ and $s$ (they are not reset in $t$).  
    One such ordered partition can be generated using \emph{part-regs} (Lines~\ref{line:fdp:allrinpermreg},\ref{line:fdp:resUres}).  
    Finally,
    $
    \breg = \{ q_0, h(x) = 3,$ $h(y)=  2, h(w) = 5, h(p) = 1, h(z) = h(s) = 4, X_{-1}, X_0, X_1, X_2, X_3 \}
    $, where 
    $X_{-1} = \{ w \}, 
    X_0 = \{ p \}, 
    X_1 = \{ z \}, 
    X_2 = \{ x, y \},$ and $
    X_3 = \{ s \}
    $.
\end{example}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Discrete_successors/discrete_successors.tex <==
\textbf{Discrete successors}~\autoref{alg:finddiscretesucc}, whose time complexity is $O(\lvert T \rvert \cdot \lvert \ackc \rvert)$, computes the discrete successors of a given region $\reg$.
In particular, a set storing the resulting discrete successors is initialized in Line~\ref{line:fdsuc:initres} and returned in Line~\ref{line:fdsuc:returnres}.  
The loop in Line~\ref{line:fdsuc:foreacht} iterates over all transitions $t$ of the original \ac{ta} that exit from the current location $q_{\reg}$ of $\reg$, identifying all possible discrete successors of $\reg$.  
If the guard $\gamma$ of $t$ is satisfied by combining the integer values of the clocks of $\reg$, as returned by \( h_{\reg} \), with their fractional parts (Line~\ref{line:fdsuc:isenabled}), a copy $\breg$ of $\reg$ is created to represent the successor region (Line~\ref{line:fdsuc:copyr}).  
The location of $\breg$ is updated to the target location $q$ of $t$ (Line~\ref{line:fdsuc:setloc}).  
The loop in Line~\ref{line:fdsuc:idxloop} iterates over all integers $-\lidx_{\breg} \le i \le \ridx_{\breg}$, enabling the inner loop in Line~\ref{line:fdsuc:setloop} to examine each clock set of $\breg$.  
If a clock $x$ is reset in $t$,
%(Line~\ref{line:fdsuc:xwasreset}), 
its integer value is set to zero (Line~\ref{line:fdsuc:setxtozero}).  
Moreover, if $x$ is either unbounded or has a nonzero fractional part (Line~\ref{line:fdsuc:hasfracpart}), it is inserted into $X_{\breg, 0}$ and removed from its previous clock set (Line~\ref{line:fdsuc:insertremovex}).  
Finally, the resulting region $\breg$ is added to the result set in Line~\ref{line:fdsuc:addtores}.

\begin{algorithm}[thb]
    \caption{\texttt{find-discrete-successors}$(\reg)$}
    \label{alg:finddiscretesucc}
    
    \KwData{$\reg$: a region.}
    \KwResult{The discrete successors of $\reg$.}
    
    \Begin() {
        $\mathit{res} \gets \varnothing$\; \label{line:fdsuc:initres}
        %\tcp{Get discrete transitions in the original \ac{ta} exiting from $q_{\reg}$}
        %$\mathcal{T} \gets \{ (q_{\reg}, a, \gamma, Y, q) \in T : a \in \act, \gamma \in \Gamma(\ackc), Y \subseteq \ackc, q \in Q \}$\;
        \ForEach{$t = (q_{\reg}, a, \gamma, Y, q) \in T$}{ \label{line:fdsuc:foreacht}
            \If{$\gamma$ is satisfied by $\reg$}{ \label{line:fdsuc:isenabled}
                $\breg \gets$ copy of $\reg$\; \label{line:fdsuc:copyr}
                $q_{\breg} \gets q$\; \label{line:fdsuc:setloc}
                \For{$i = -\lidx_{\breg}$ \KwTo $\ridx_{\breg}$}{ \label{line:fdsuc:idxloop}
                    \ForEach{$x \in X_{\breg,i}$ such that $x \in Y$}{ \label{line:fdsuc:setloop}
                        %\If{$x \in Y$}{ \label{line:fdsuc:xwasreset}
                            $h_{\breg}(x) \gets 0$\; \label{line:fdsuc:setxtozero}
                            \If{$i \neq 0$}{ \label{line:fdsuc:hasfracpart}
                                $X_{\breg,0} \gets X_{\breg,0} \cup \{x\}$;
                                $X_{\breg,i} \gets X_{\breg,i} \setminus \{x\}$\; \label{line:fdsuc:insertremovex}
                         %   }
                        }
                    }
                }
                % Non dovrebbe più servire togliere esplicitamente gli insiemi vuoti perchè hai già detto nella sezione 3 che gli insiemi vuoti sono omessi in automatico
                %\For{$i = -\lidx_{\breg}$ \KwTo $\ridx_{\breg}$}{
                %\If{$X_{\breg,i} = \varnothing$ and $i \neq 0$}{
                %        remove $X_{\breg, i}$ from $\breg$\;
                        %\texttt{remove}$(\breg, i)$\;
                %    }
                %}
                $\mathit{res} \gets \mathit{res} \cup \{ \breg \}$\; \label{line:fdsuc:addtores}
            }
        }
        \Return $\mathit{res}$\; \label{line:fdsuc:returnres}
    }
\end{algorithm}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/Figures/delaypredexamplecropped.tex <==
\renewcommand{\arraystretch}{1}
\definecolor{lightgray}{gray}{0.95}
\begin{figure}[tb]
    \centering

    % Left: actual figure
    \begin{subfigure}[H]{0.54\textwidth}
        \centering
        \includegraphics[width=\linewidth]{DelayAndDiscretePredecessors/Figures/delaypredexamplecrop.pdf}
        \caption{Partial computation of delay predecessors of $\reg_0$.}
        \label{fig:partcompfig}
    \end{subfigure}%
    %
    \hfill
    %    
    %Right: table displayed as a subfigure
    \begin{subfigure}[H]{0.44\textwidth}
        \centering
        %\rowcolors{2}{lightgray}{white}
       \rowcolors{2}{lightgray}{white}  % alternating row colors
        \begin{tabular}{
        >{\centering\arraybackslash}p{1.3cm}  % Region column
        >{\centering\arraybackslash}p{1.3cm}  % Class column
        p{2cm}                              % Unbounded column
        }
        \toprule
        \textbf{Region} & \textbf{Class} & \textbf{Unbounded} \\
        \midrule
        $\reg_0$ & $\cu$ & yes, $\{x, y\}$ \\
        $\reg_1$ & $\ca$ & yes, $\{y\}$ \\
        $\reg_2$ & $\cb$ & yes, $\{y\}$ \\
        $\reg_3$ & $\ca$ & yes, $\{y\}$ \\
        $\reg_4$ & $\ca$ & no, $\varnothing$ \\
        $\reg_5$ & $\cc$ & no, $\varnothing$ \\
        $\reg_6$ & $\cb$ & yes, $\{y\}$ \\
        $\reg_7$ & $\ca$ & yes, $\{y\}$ \\
        $\reg_8$ & $\ca$ & no, $\varnothing$ \\
        $\reg_9$ & $\cc$ & no, $\varnothing$ \\
        \bottomrule
        \end{tabular}
        \caption{Table listing regions $\reg_i$, $0 \le i \le 9$, their class, and their unbounded clocks (if any).}
        \label{fig:partcomptab}
    \end{subfigure}

    \caption{Example of delay predecessors computation from $\reg_0$ (left), stopped upon reaching bounded regions, and a table with additional information about the regions (right).
    Triangles symbolically represent entire regions rather than specific points within them.}
    \label{fig:partcomb}
\end{figure}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/delay_and_discrete_predecessors.tex <==
We present algorithms computing discrete successors and immediate delay predecessors regions.
For brevity, immediate delay successors and discrete predecessors algorithms are deferred to the Appendix in \autoref{app:foreword_delay_successors_algorithm} and \autoref{app:discrete_predecessors_algorithm}.

\input{DelayAndDiscretePredecessors/Discrete_successors/discrete_successors}

\input{DelayAndDiscretePredecessors/Delay_Predecessors/delay_predecessors}

% \subsubsection{Discrete predecessors}
% \input{DelayAndDiscretePredecessors/Discrete Predecessors/discrete_predecessors}


==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/DelayAndDiscretePredecessors/production_cell.tex <==
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[
	->,
	>=stealth',
	shorten >=2pt, 
	auto,
    transform shape,
    align=center,
    scale=0.77,
    state/.style={thick, circle, draw, minimum size=1.3cm}
    ] 
    
    \node[
          state,
          initial,
          initial text =,
          label=above left:$\mathbf{c}$
         ] 
         (q0) {$\mathit{feed}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          right = 4.6cm of q0
         ] 
         (q1) {$\mathit{table}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          right = 4.6cm of q1
         ] 
         (q2) {$\mathit{robot_p}$};

    \node[
          state,
          label=above left:$\mathbf{c}$,
          above = 2.8cm of q2
         ] 
         (q3) {$\mathit{press}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          left = 4.6cm of q3
         ] 
         (q4) {$\mathit{robot_d}$};
	
    \node[
          state,
          label=above left:$\mathbf{c}$,
          left = 4.6cm of q4
         ] 
         (q5) {$\mathit{depot}$};

    \node[
          state,
          label=above left:$\mathbf{e}$,
          left = 0cm of q2,
          yshift=2.7cm
         ] 
         (q6) {$\mathit{fall_p}$};

    \node[
          state,
          label=above left:$\mathbf{e}$,
          right = 0cm of q0,
          yshift=2.7cm
         ] 
         (q7) {$\mathit{fall_d}$};

	\draw [line width=0.35mm] 
    
	(q0) 
    edge 
    node[above, pos=0.6]{$\mathit{toTable}$ \\ $x = 2$} 
    node[below, pos=0.6]{$\resetClock{x}$}
    (q1)
	
    (q1) 
    edge 
    node[above, pos=0.4]{$\mathit{takePlate_p}$ \\ $x \ge 1 \land x \le 3$} 
    node[below, pos=0.4]{$\resetClock{x}$}
    (q2)

    (q2) 
    edge 
    node[right]{$\mathit{toPress}$ \\ $x \ge 2 \land x \le 4$ \\ $\resetClock{x}$}
    (q3)

    (q3) 
    edge 
    node[above]{$\mathit{takePlate_d}$ \\ $x \ge 3 \land x \le 5$} 
    node[below]{$\resetClock{x}$}
    (q4)

    (q4) 
    edge 
    node[above]{$\mathit{toDepot}$ \\ $x \ge 3 \land x \le 6$} 
    node[below]{$\resetClock{x}$}
    (q5)

    (q2) 
    edge 
    node[left, xshift=-9pt]{$\mathit{toPress}$ \\ $x < 2$ \\ $\resetClock{x}$}
    (q6)

    (q4) 
    edge %[out=270, in=0]
    node[right, pos=0.4, xshift = -12pt, yshift=-20pt]{$\mathit{toDepot}$ \\ $x \ge 4$ \\ $\resetClock{x}$}
    (q7)

    (q6) 
    edge [out=180, in=15]
    node[right, pos=0.5, xshift=22pt]{$\mathit{restore_p}$ \\ $x > 1 \land x < 2$}
    (q0)

    (q7) 
    edge
    node[right, pos=0.4, xshift=-2pt]{$\mathit{restore_d}$ \\ $x > 1 \land x \le 5$}
    (q0)

    (q5) 
    edge 
    node[left]{ $\mathit{newPlate}$ \\ $\resetClock{x}$}
    (q0)
	;
\end{tikzpicture}
\end{center}
\caption{A \ac{ta} modeling a Production Cell.
The passage of time is tracked by a clock $y$, which is neither reset nor used in any guard, and is therefore omitted from the figure.}
\label{fig:production_cell_text}
\end{figure}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/Benchmark_Tables/backward_tables.tex <==
%\begin{table}[thb]
%\centering
%\caption{Forward and backward reachability for both \flower{} and a single \ac{ta} version of \fischer{}.}
%\label{tab:backward_scalability}
%{\setlength{\tabcolsep}{1.75pt}
%\begin{tabular}{c | r r | r r}
%\toprule
%\multirow{2}{*}{\textbf{K}} & \multicolumn{2}{c|}{\textbf{Forward}} & \multicolumn{2}{c}{\textbf{Backward}} \\
%%& \multicolumn{1}{c}{\textbf{VT}} 
%& \multicolumn{1}{c|}{\textbf{Regions}} 
%& \multicolumn{1}{c}{\textbf{VT}}
%& \multicolumn{1}{c}{\textbf{Regions}} \\
%\midrule
%
%
% FLOWER DATA
%\multicolumn{5}{c}{$\blacktriangleright$ {\normalsize \flower{}}~\cite{J_rgensen_2012} :: reachability %$\blacktriangleleft$} \\
%\midrule
%\rowcolor{white} 11     & \textbf{0.031}         & \textbf{30761}     & 0.060         & 38669      \\
%\rowcolor{lightgray} 13 & \textbf{0.404}         & \textbf{370331}    & 0.615         & 388911     \\
%\rowcolor{white} 15     & \textbf{7.014}         & \textbf{5142671}   & 9.414         & 4921043    \\
%\rowcolor{lightgray} 17 & \textbf{16.071}        & \textbf{11023829}  & 21.497        & 11077295   \\
%\midrule
%
%
% FISCHER DATA
%\multicolumn{5}{c}{$\blacktriangleright$ {\normalsize \fischer{}}~\cite{tarzan2025} :: unreachability %$\blacktriangleleft$} \\
%\midrule
%\rowcolor{white} 3  & 0.007         & 9083      & $\boldsymbol{\varepsilon}$ & \textbf{264}        \\
%\rowcolor{lightgray} 4      & 0.141         & 183459    & \textbf{0.001}         & \textbf{1316}       \\
%\rowcolor{white} 5  & 4.061         & 4182681   & \textbf{0.008}         & \textbf{8724}       \\
%\rowcolor{lightgray} 6      & OOM           & OOM       & \textbf{0.100}         & \textbf{77084}      \\
%\midrule
%
%
%\multicolumn{5}{c}{$\blacktriangleright$ {\normalsize \train{}} :: reachability / unreachability %$\blacktriangleleft$} \\
%\midrule
% TrainAHV Flat 2 reachable
%\rowcolor{white} 4 & 0.001 & 888 & 3.695 & 3426821 \\
%
% TrainAHV Flat 3 reachable
%\rowcolor{lightgray} 5 & 0.074 & 89834 & OOM & OOM \\
%
%\midrule[0.5pt]
%
% TrainAHV Flat 2 efficient (unreachable)
%\rowcolor{white} 4 &0.016 & 17124 & 0.030 & 26914 \\
%
% TrainAHV Flat 3 efficient (unreachable)
%\rowcolor{lightgray} 5 & 0.866 & 912597 & 0.618 & 614220 \\
%\bottomrule
%\end{tabular}%
%}
%\end{table}
%
%
%
\begin{table}[tb]
\centering
\caption{Backward reachability results. \fischer{} goes out of memory at $K=6$. Tests use \ac{dfs} except \train{}, for which \ac{bfs} is faster. \flower{} checks reachability, \fischer{} unreachability, and \train{} reachability (rows 1,2) and unreachability (rows 3,4).}
\label{tab:backward_scalability}
{\setlength{\tabcolsep}{2.25pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{r r | r r !{\vrule width 1pt} r r | r r !{\vrule width 1pt} r r | r r}
\toprule
\multicolumn{4}{c!{\vrule width 1pt}}
{$\blacktriangleright$ {\normalsize {\flower{}}~\cite{J_rgensen_2012}} :: DFS $\blacktriangleleft$} & 
\multicolumn{4}{c!{\vrule width 1pt}}
{$\blacktriangleright$ {\normalsize {\fischer{}}~\cite{tarzan2025}} :: DFS $\blacktriangleleft$} & 
\multicolumn{4}{c}
{$\blacktriangleright$ {\normalsize{\train{}}~\cite{tarzan2025}} :: BFS $\blacktriangleleft$} \\
\midrule
\multicolumn{2}{c|}{\makecell{\emph{Forward}\\$K = 11,13,15,17$}}
& \multicolumn{2}{c!{\vrule width 1pt}}{\makecell{\emph{Backward}\\$K = 11,13,15,17$}}
& \multicolumn{2}{c|}{\makecell{\emph{Forward}\\$K = 3,4,5,6$}}
& \multicolumn{2}{c!{\vrule width 1pt}}{\makecell{\emph{Backward}\\$K = 3,4,5,6$}}
& \multicolumn{2}{c|}{\makecell{\emph{Forward}\\$K = 4,5,4,5$}}
& \multicolumn{2}{c}{\makecell{\emph{Backward}\\$K = 4,5,4,5$}} \\
\multicolumn{1}{c}{\textbf{VT}} 
& \multicolumn{1}{c|}{\textbf{Regions}}
& \multicolumn{1}{c}{\textbf{VT}}
& \multicolumn{1}{c!{\vrule width 1pt}}{\textbf{Regions}}
& \multicolumn{1}{c}{\textbf{VT}}
& \multicolumn{1}{c|}{\textbf{Regions}}
& \multicolumn{1}{c}{\textbf{VT}}
& \multicolumn{1}{c!{\vrule width 1pt}}{\textbf{Regions}} 
& \multicolumn{1}{c}{\textbf{VT}}
& \multicolumn{1}{c|}{\textbf{Regions}}
& \multicolumn{1}{c}{\textbf{VT}} 
& \multicolumn{1}{c}{\textbf{Regions}} \\
\midrule
%
\rowcolor{white} 0.028 & 30761 & 0.060 & 38669 & 0.007 & 9083 & $\varepsilon$ & 264 & $\varepsilon$ & 1241 & 0.171 & 118868 \\
\rowcolor{lightgray} 0.412 & 370331 & 0.615 & 388911 & 0.141 & 183459 & 0.001 & 1316 & 0.026 & 31516 & 66.877 & 31051667 \\

\hhline{~~~~~~>{\arrayrulecolor{black}}~~---->{\arrayrulecolor{black}}}

\rowcolor{white} 7.188 & 5142671 & 9.414 & 4921043 & 4.061 & 4182681 & 0.008 & 8724 & 0.013 & 17124 & 0.030 & 26914 \\
\rowcolor{lightgray} 16.212 & 11023829 & 21.497 & 11077295 & --- & --- & 0.100 & 77084 & 1.000 & 912597 & 0.635 & 614220 \\
\bottomrule
\end{tabular}%
}
}
\end{table}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/Benchmark_Tables/big_constants.tex <==
\definecolor{lightgray}{gray}{0.95}
\setlength{\aboverulesep}{1pt}
\setlength{\belowrulesep}{1pt}
{\renewcommand{\arraystretch}{0.95}
{\setlength{\tabcolsep}{3.25pt}
\begin{table}[tb]
\centering
\caption{Large constants negatively impact the \ac{vt} of regions, unlike zones.
Here, the first row of \pagerank{} corresponds to the variant with truncated constants.}
\label{tab:constants}
\resizebox{\textwidth}{!}{
\begin{tabular}{%
    c|rrrr|rrrr|rrrr
}
\toprule
\multirow{2}{*}{\textbf{K}}
  & \multicolumn{4}{c|}{\textbf{TARZAN}}
  & \multicolumn{4}{c|}{\textbf{TChecker}}
  & \multicolumn{4}{c}{\textbf{UPPAAL}} \\
%
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{Regions}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{States}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c}{\textbf{States}} \\
\midrule
% ----------------------- CSMA DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \csma{}}~\cite{kiviriga2021randomized} ::
[Query: $\exists \Diamond \left( \parbox{7.5cm}{\begin{math}P_1.\mathit{senderRetry} \land P_2.\mathit{senderRetry} \land P_3.\mathit{senderTransm} \end{math} \\ \begin{math}\land \; P_4.\mathit{senderRetry} \land \dots \land P_7.\mathit{senderRetry}\end{math}} \right)$]
$\blacktriangleleft$} \\
\midrule
\rowcolor{white}
21  & 0.198 & 0.215 & 364.96 & 20936
   & 0.004 & 0.038 & 30.32 & 232
   & \textbf{0.001} & \textbf{0.061} & \textbf{20.24} & \textbf{269} \\
%\rowcolor{lightgray}
%22N  & 0.262 & 0.281 & 482.81 & 25422
%   & 0.006 & 29.006 & 40.22 & 78
%   & 0.001 & 0.061 & 20.10 & 24 \\
%\rowcolor{white}
%25N  & 0.388 & 0.409 & 700.02 & 32931
%   & 0.009 & 61.097 & 61.51 & 84
%   & 0.002 & 0.062 & 20.64 & 27 \\
\rowcolor{lightgray}
31  & 0.674 & 0.701 & 1194.45 & 47526
   & 0.018 & 0.218 & 117.03 & 371
   & \textbf{0.002} & \textbf{0.064} & \textbf{21.11} & \textbf{554} \\
\rowcolor{white}
51  & 3.364 & 3.431 & 5351.35 & 131906
   & 0.293 & 1.386 & 837.12 & 1381
   & \textbf{0.010} & \textbf{0.077} & \textbf{23.89} & \textbf{1424} \\
\midrule
% ----------------------- PAGERANK DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \pagerank{}}~\cite{Baresi2020} ::
[Query: $\exists \Diamond ( \mathit{Stage}_7.\mathit{Completed} )$]
$\blacktriangleleft$} \\
\midrule
\rowcolor{white}
9  & 0.068 & 0.085 & 179.33 & 4193
   & 0.002 & 0.086 & 58.54 & 1129
   & \textbf{0.002} & \textbf{0.076} & \textbf{22.89} & \textbf{1129} \\
\rowcolor{lightgray}
9  & 4.227 & 4.361 & 10950.36 & 257311
   & 0.002 & 0.085 & 58.53 & 1129
   & \textbf{0.002} & \textbf{0.076} & \textbf{23.01} & \textbf{1129} \\
\bottomrule
\end{tabular}
}
\end{table}
}
}


==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/Benchmark_Tables/closed_ta.tex <==
\definecolor{lightgray}{gray}{0.95}
\setlength{\aboverulesep}{1pt}
\setlength{\belowrulesep}{1pt}
{\renewcommand{\arraystretch}{0.95}
{\setlength{\tabcolsep}{3.25pt}
\begin{table}[tb]
\centering
\caption{The results are derived from networks of closed \acp{ta}, where guards may either be punctual or contain non-strict inequalities.
In this setting, \toolname{} can handle both large networks (\medical{}) and large constants (\mpeg{}).}
\label{tab:closed}
\resizebox{\textwidth}{!}{
\begin{tabular}{%
    c|rrrr|rrrr|rrrr
}
\toprule
\multirow{2}{*}{\textbf{K}}
  & \multicolumn{4}{c|}{\textbf{TARZAN}}
  & \multicolumn{4}{c|}{\textbf{TChecker}}
  & \multicolumn{4}{c}{\textbf{UPPAAL}} \\
%
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{Regions}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{States}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c}{\textbf{States}} \\
\midrule
% ----------------------- MEDICALWORKFLOW DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \medical{}}~\cite{tapaal2025} ::
[Query: $\exists \Diamond ( \mathit{Patient}_1.\mathit{Done} \land \mathit{Patient}_2.\mathit{Done} \land \dots \land \mathit{Patient}_{K - 2}.\mathit{Done} ) $]
$\blacktriangleleft$} \\
\midrule
\rowcolor{white}
12  & 0.007 & 0.021 & 33.39 & 660
   & 0.011 & 0.030 & 22.63 & 639
   & \textbf{0.002} & \textbf{0.059} & \textbf{20.83} & \textbf{582} \\
\rowcolor{lightgray}
22  & 0.056 & 0.072 & 204.97 & 2715
   & 0.316 & 0.560 & 173.75 & 3774
   & \textbf{0.032} & \textbf{0.093} & \textbf{31.76} & \textbf{2862} \\
\rowcolor{white}
42  & \textbf{0.609} & \textbf{0.647} & \textbf{2271.65} & \textbf{15025}
   & 13.571 & 16.096 & 2517.18 & 25544
   & 1.275 & 1.379 & 230.07 & 16522 \\
\rowcolor{lightgray}
72  & \textbf{5.781} & \textbf{5.959} & \textbf{12891.17} & \textbf{68990}
   & 355.827 & 389.223 & 16109.45 & 126949
   & 54.200 & 54.838 & 2799.57 & 74762 \\
\rowcolor{white}
102  & \textbf{27.918} & \textbf{28.466} & \textbf{13780.57} & \textbf{189555}
   & KO & KO & KO & KO
   & 593.317 & 597.306 & 12364.67 & 202302 \\
\midrule
% ----------------------- MPEG2 DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \mpeg{}}~\cite{tapaal2025} ::
[Query: $\exists \Diamond ( \mathit{BFrame}_1.\mathit{Bout} \land \mathit{BFrame}_2.\mathit{Bout} \land \dots \land \mathit{BFrame}_{K - 4}.\mathit{Bout} )$]
$\blacktriangleleft$} \\
\midrule
\rowcolor{white}
8  & 0.365 & 0.385 & 451.46 & 26916
   & 0.003 & 0.014 & 8.96 & 531
   & \textbf{0.001} & \textbf{0.058} & \textbf{19.46} & \textbf{537} \\
\rowcolor{lightgray}
12  & \textbf{0.796} & \textbf{0.819} & \textbf{718.63} & \textbf{27238}
   & 8.405 & 8.663 & 252.70 & 383103
   & 1.621 & 1.766 & 112.33 & 383109 \\
\rowcolor{white}
16  & \textbf{1.364} & \textbf{1.392} & \textbf{1032.46} & \textbf{27704}
   & --- & TO & --- & ---
   & --- & TO & --- & --- \\
\bottomrule
\end{tabular}
}
\end{table}
}
}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/Benchmark_Tables/full_state_space.tex <==
\definecolor{lightgray}{gray}{0.95}
\setlength{\aboverulesep}{1pt}
\setlength{\belowrulesep}{1pt}
{\renewcommand{\arraystretch}{0.95}
{\setlength{\tabcolsep}{3.25pt}
\begin{table}[t]
\centering
\caption{Safety properties require \toolname{} to visit the entire reachable state space.}
\label{tab:safety}
\resizebox{\textwidth}{!}{
\begin{tabular}{%
    c|rrrr|rrrr|rrrr
}
\toprule
\multirow{2}{*}{\textbf{K}}
  & \multicolumn{4}{c|}{\textbf{TARZAN}}
  & \multicolumn{4}{c|}{\textbf{TChecker}}
  & \multicolumn{4}{c}{\textbf{UPPAAL}} \\
%
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{Regions}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{States}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c}{\textbf{States}} \\
\midrule
% ----------------------- FISCHER DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \fischer{}}~\cite{uppaalSite} ::
[Query: $\exists \Diamond ( \mathit{Fischer}_1.\mathit{cs} \land \mathit{Fischer}_2.\mathit{cs} ) $]
$\blacktriangleleft$} \\
\midrule
%\rowcolor{white}
%2  & 0.001 & 0.015 & 9.60 & 542
%   & $\varepsilon$ & 0.005 & 5.70 & 18
%   & 0.001 & 0.055 & 18.87 & 18 \\
%\rowcolor{lightgray}
%3  & 0.025 & 0.039 & 55.62 & 9324
%   & $\varepsilon$ & 0.006 & 5.77 & 65
%   & 0.001 & 0.055 & 18.91 & 65 \\
\rowcolor{white}
4  & 0.644 & 0.669 & 1098.36 & 180032
   & $\boldsymbol{\varepsilon}$ & \textbf{0.007} & \textbf{6.75} & \textbf{220}
   & 0.001 & 0.055 & 18.96 & 220 \\
\rowcolor{lightgray}
5  & 19.627 & 19.849 & 12948.99 & 3920652
   & 0.004 & 0.011 & 9.30 & 727
   & \textbf{0.002} & \textbf{0.057} & \textbf{19.07} & \textbf{727} \\
\rowcolor{white}
6  & --- & --- & OOM & ---
   & 0.024 & 0.032 & 12.25 & 2378
   & \textbf{0.008} & \textbf{0.064} & \textbf{19.43} & \textbf{2378} \\
\bottomrule
\end{tabular}
}
\end{table}
}
}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/Benchmark_Tables/punctual_guards.tex <==
\definecolor{lightgray}{gray}{0.95}
\definecolor{lightgreen}{RGB}{210,255,190}
\setlength{\aboverulesep}{1pt}
\setlength{\belowrulesep}{1pt}
{\renewcommand{\arraystretch}{0.95}
{\setlength{\tabcolsep}{3.25pt}
\begin{table}[tb]
\centering
\caption{When all transitions have punctual guards, regions may outperform zones.
Here, \flower{} is a single \ac{ta}, while the others are networks of \ac{ta}.}
\label{tab:punctual}
\resizebox{\textwidth}{!}{
\begin{tabular}{%
    c|rrrr|rrrr|rrrr
}
\toprule
\multirow{2}{*}{\textbf{K}}
  & \multicolumn{4}{c|}{\textbf{TARZAN}}
  & \multicolumn{4}{c|}{\textbf{TChecker}}
  & \multicolumn{4}{c}{\textbf{UPPAAL}} \\
%
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{Regions}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c|}{\textbf{States}}
  & \multicolumn{1}{c}{\textbf{VT}}
  & \multicolumn{1}{c}{\textbf{ET}}
  & \multicolumn{1}{c}{\textbf{Mem}}
  & \multicolumn{1}{c}{\textbf{States}} \\
\midrule
% ----------------------- BOOLEAN DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \boolea{}}~\cite{tarzan2025} ::
[Query: $\exists \Diamond( \mathit{ctr}_1 = 1 \land \mathit{ctr}_2 = 1 \land \dots \land \mathit{ctr}_K = 1 )$]
$\blacktriangleleft$} \\
\midrule
%\rowcolor{white}
%2  & $\varepsilon$ & 0.013 & 7.62 & 9
%   & $\varepsilon$ & 0.005 & 5.70 & 5
%   & $\varepsilon$ & 0.051 & 18.80 & 4 \\
\rowcolor{white}
4  & $\varepsilon$ & 0.013 & 7.78 & 24
   & $\boldsymbol{\varepsilon}$ & \textbf{0.007} & \textbf{6.47} & \textbf{185}
   & 0.001 & 0.052 & 18.85 & 185 \\
\rowcolor{lightgray}
6  & \textbf{0.003} & \textbf{0.016} & \textbf{13.42} & \textbf{425}
   & 0.088 & 0.096 & 13.80 & 8502
   & 0.075 & 0.128 & 19.91 & 8502 \\
\rowcolor{white}
8  & \textbf{0.013} & \textbf{0.027} & \textbf{29.10} & \textbf{1009}
   & 75.461 & 75.980 & 220.82 & 566763
   & 77.204 & 77.523 & 81.79 & 566763 \\
\midrule
% ----------------------- FLOWER DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \flower{}}~\cite{J_rgensen_2012} :: 
[Query: $\exists \Diamond ( \mathit{Flower.Goal} )$]
$\blacktriangleleft$} \\
\midrule
%\rowcolor{white}
%2  & $\varepsilon$ & 0.013 & 7.64 & 13
%   & $\varepsilon$ & 0.006 & 5.73 & 6
%   & $\varepsilon$ & 0.055 & 18.80 & 5 \\
\rowcolor{white}
5  & ${\boldsymbol \varepsilon}$ & \textbf{0.013} & \textbf{7.92} & \textbf{95}
   & 0.001 & 0.007 & 6.35 & 150
   & 0.001 & 0.056 & 18.82 & 150 \\
\rowcolor{lightgray}
7  & $\boldsymbol{\varepsilon}$ & \textbf{0.022} & \textbf{10.65} & \textbf{573}
   & 0.322 & 0.330 & 13.12 & 3508
   & 0.399 & 0.455 & 19.76 & 3508 \\
\rowcolor{white}
9  & \textbf{0.007} & \textbf{0.022} & \textbf{58.62} & \textbf{9161}
   & --- & TO & --- & ---
   & --- & TO & --- & --- \\
\midrule
% ----------------------- GATES DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \gates{}}~\cite{tarzan2025} ::
[Query: $\exists \Diamond ( \mathit{Unlocker.Goal} )$]
$\blacktriangleleft$} \\
\midrule
%\rowcolor{white}
%2  & $\varepsilon$ & 0.013 & 7.79 & 26
%   & $\varepsilon$ & 0.005 & 5.70 & 16
%   & $\varepsilon$ & 0.054 & 18.86 & 15 \\
\rowcolor{white}
5  & $\boldsymbol{\varepsilon}$ & \textbf{0.013} & \textbf{8.84} & \textbf{76}
   & 0.001 & 0.008 & 7.19 & 549
   & 0.001 & 0.055 & 19.01 & 549 \\
\rowcolor{lightgray}
7  & $\boldsymbol{\varepsilon}$ & \textbf{0.014} & \textbf{11.23} & \textbf{151}
   & 0.110 & 0.122 & 21.08 & 32979
   & 0.035 & 0.092 & 22.79 & 32979 \\
\rowcolor{white}
9  & \textbf{0.001} & \textbf{0.015} & \textbf{15.43} & \textbf{251}
   & 47.895 & 48.771 & 806.72 & 3071646
   & 5.228 & 6.509 & 451.71 & 3071646 \\
\midrule
% ----------------------- RING DATASET -----------------------
\multicolumn{13}{c}{$\blacktriangleright$
{\normalsize \ring{}}~\cite{tarzan2025} ::
[Query: $\exists \Diamond ( P_0.\mathit{Goal} \land P_1.\mathit{Goal} \land ... \land P_K.\mathit{Goal} )$]
$\blacktriangleleft$} \\
\midrule
%\rowcolor{white}
%2  & $\varepsilon$ & 0.013 & 7.84 & 59
%   & $\varepsilon$ & 0.006 & 5.77 & 41
%   & $\varepsilon$ & 0.054 & 18.83 & 40 \\
\rowcolor{white}
4  & \textbf{0.001} & \textbf{0.015} & \textbf{12.40} & \textbf{542}
   & 0.020 & 0.029 & 11.56 & 7738
   & 0.010 & 0.065 & 19.52 & 7738 \\
\rowcolor{lightgray}
6  & \textbf{0.011} & \textbf{0.025} & \textbf{48.96} & \textbf{3397}
   & 12.137 & 12.561 & 268.93 & 1180575
   & 3.406 & 3.715 & 128.87 & 1180575 \\
\rowcolor{white}
8  & \textbf{0.204} & \textbf{0.225} & \textbf{687.77} & \textbf{47063}
   & --- & TO & --- & ---
   & --- & TO & --- & --- \\
\bottomrule
\end{tabular}
}
\end{table}
}
}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/backward_reachability.tex <==
%We begin the evaluation of backward reachability by considering the \flower{} \ac{ta}, depicted in \autoref{fig:flower_main_text}.
We begin with a backward unreachability example on \flower{}, and then compare its forward and backward reachability results.
The entire \flower{} reachable state space, when considering five clocks and computed going forward starting from the initial region
$
\reg_0 = \{ q_0, h(x_1) = h(x_2) = h(x_3) = h(x_4) = h(y) = 0, X_0 \}$, where $X_{\reg_0, 0} = \{ x_1, x_2, x_3, x_4, y \}
$, resulted in 1517 regions, computed in 1.18 ms.

%Since tracking the order in which clocks become unbounded yields a finer partitioning of the state space, backward reachability may explore more regions than those appearing in the entire state space computed going forward.
%
%We first demonstrate that the backward reachability algorithms implemented in \toolname{} correctly identify an initial region as reachable when starting from a region reached through forward exploration. Consider the reachability query
%$\exists \Diamond \mathit{Flower.Goal}$.
%The region reached with forward reachability starting from $\reg_0$ is
%$
%\reg_1 = \{ \mathit{Goal}, h(x_1) = h(x_2) = h(x_3) = h(x_4) = 0, h(y) = 1, X_{-1}, X_0 \}$, where 
%$X_{\reg_1, -1} = \{ y \}$ and $X_{\reg_1, 0} = \{ x_1, x_2, x_3, x_4 \}
%$.
%Reaching $\reg_1$ required computing 95 regions in 0.062 ms.
%Starting from $\reg_1$, the backward reachability algorithm successfully reaches the initial region $\reg_0$, computing %167 regions in 0.185 ms.
%
%A similar experiment was performed starting from an arbitrary region, such as
%$
%\reg_2 = \{ q_0, h(x_1) = 1, h(x_2) = 2, h(x_3) = h(x_4) = 0, h(y) = 1, X_{-1}, X_0 \}$, where 
%$X_{\reg_2, -1} = \{ y \}$ and $X_{\reg_2, 0} = \{ x_1, x_2, x_3, x_4 \}
%$.
%Region \(\reg_2\) is reachable; for instance, it can be obtained by first resetting $x_3$ and then $x_4$ from the %reachable region
%$
%\reg_3 = \{ q_0, h(x_1) = 1, h(x_2) = 2, h(x_3) = 3, h(x_4) = 4, h(y) = 1, X_{-1}, X_0 \}$, where 
%$X_{\reg_3, -1} = \{ y \}$ and $X_{\reg_3, 0} = \{ x_1, x_2, x_3, x_4 \}
%$.
%In this case, reaching $\reg_0$ from $\reg_2$ required computing 197 regions in 0.190 ms.
%
%Next, 

Backward reachability can offer a practical advantage for proving unreachability, since it may avoid a complete state space exploration.
Consider the region
$
\reg_1 = \{ q_0, h(x_1) = 1, h(x_2) = 2, h(x_3) = h(x_4) = 0, h(y) = 1, X_{-1}, X_0 \}$, where 
$X_{\reg_1, -1} = \{ x_2, y \}$ and $X_{\reg_1, 0} = \{ x_1, x_3, x_4 \}
$.
$\reg_1$ is unreachable: it requires both $x_2$ and $y$ to become unbounded simultaneously, but the constraint $y \ge 1$ forces $y$ to become unbounded before $x_2$.
\toolname{} classifies $\reg_1$ as unreachable by verifying that $\reg_0$ is unreachable from $\reg_1$, requiring 272 regions in 0.245 ms.
By adjusting $\reg_1$ with the correct ordering in which clocks become unbounded, we obtain
$
\reg_2 = \{ q_0, h(x_1) = 1, h(x_2) = 2, h(x_3) = h(x_4) = 0, h(y) = 1, X_{-2}, X_{-1}, X_0 \}$, where 
$X_{\reg_2, -2} = \{ x_2 \}$, $X_{\reg_2, -1} = \{ y \}$, and $X_{\reg_2, 0} = \{ x_1, x_3, x_4 \}
$.
Region $\reg_2$ is reachable.
Reaching $\reg_0$ from $\reg_2$ required 263 regions in 0.378 ms.

Now, consider the version of \flower{} with $K = n + 1$ clocks.  
Let $\reg_K$ denote the region in location $\mathit{Goal}$ in which all clocks $x_i$ are exactly equal to zero (no fractional part) and $y \ge 1$ holds. %, and $q = \mathit{Goal}$.  
\autoref{tab:backward_scalability} reports the \ac{vt} and number of regions stored by \toolname{} when checking the forward and backward reachability of $\reg_K$.
The results show that forward reachability is generally faster and requires fewer regions, while backward reachability remains comparable \Red{in this setting}.

\input{Implementation_and_Experimental_Evaluation/Benchmark_Tables/backward_tables}

Backward reachability was employed to verify that in \fischer{} two processes cannot occupy the critical section simultaneously.
As backward reachability does not currently support networks of \ac{ta} nor integer variables, we developed a script to construct a single \ac{ta} version of \fischer{}~\cite{tarzan2025}, in which the \emph{pid} variable is directly encoded within its locations.
The safety property to be verified with $K$ processes is described as follows: processes $1$ through $K-2$ are requesting access to the critical section, with their clocks strictly between $1$ and $2$; processes $K-1$ and $K$ are both in the critical section, with their clocks greater than $2$; \emph{pid} is equal to $K$.
A preliminary phase was necessary to compute the initial subset of regions from which backward reachability was started. 
This required considering all ordered partitions of the fractional parts of bounded clocks as well as all ordered partitions of unbounded clocks.
\Red{Clock constraints in the property were introduced to enable the manual computation of this subset.}
Backward reachability results, reported in \autoref{tab:backward_scalability}, demonstrate superior performance compared to forward reachability, \Red{to the extent that an out-of-memory event becomes feasible}.
\Red{Indeed, the unreachable portion of the state space limited the backward exploration to a relatively small number of regions.}
We evaluated the same property with Uppaal (which uses forward reachability) on the same \fischer{} model and obtained:
for $K=3$, 88 states in 0.001 s;
for $K=4$, 460 states in 0.004 s;
for $K=5$, 2765 states in 0.025 s;
and for $K=6$, 19042 states in 0.214 s.
In this comparison, \toolname{} outperformed Uppaal when using backward reachability.

Backward reachability was also applied to \train{}~\cite{tarzan2025} (we developed a script to convert it into a single \ac{ta} version).
Exploration was conducted in \ac{bfs}, as it achieved better performance on this model.
\train{} allows two or more trains to be in the crossing while the gate is down.
Rows 1,2 of \autoref{tab:backward_scalability} report the results for (i) reaching the first region detected by the \ac{bfs} exploration in which at least two trains occupy the crossing while the gate is down, and (ii) computing the backward predecessors from this region to an initial one. 
In this case, backward reachability requires substantially more regions than forward reachability.
We also verified the safety property stating that whenever a train is in the crossing, the number of trains in the crossing cannot be zero (\emph{i.e.}, no counter malfunction).
Such property with $K-2$ trains, a gate, and a controller, is described as follows: trains $1$ to $K-3$ are not in the crossing and their clocks are strictly between $2$ and $3$; train $K-2$ is in the crossing and its clock is exactly $4$; the gate's clock is strictly between $1$ and $2$, and the controller's clock is greater than $1$. 
As in \fischer{}, we first explicitly identified the initial subset of regions from which backward reachability was started. 
Rows 3,4 of \autoref{tab:backward_scalability} show that, in this case, forward and backward reachability perform comparably.

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/figures/flower.tex <==
\setlength{\intextsep}{0pt}
\begin{wrapfigure}[12]{r}{0.35\textwidth}
\centering
\captionsetup{skip=5pt}
\begin{tikzpicture}[
    ->,
    >=stealth',
    shorten >=2pt, 
    auto,
    transform shape,
    align=center,
    scale=0.865,
    state/.style={thick, circle, draw, minimum size=1cm}
] 
\useasboundingbox (-2, -3.1) rectangle (2.9, 1.71);

  % Main state
  \node[state, accepting] (q) {$q_0$};
  % Goal state below
  \node[state, below of=q, yshift=-1.5cm] (goal) {$\mathit{Goal}$};
  % Ellipsis to suggest more loops (slightly above q)
  \node[above=1cm of q, xshift=23pt, yshift=-37pt] (dots) {\Large $\mathbf{\cdots}$};
  \draw [thick] 
  % Edges and loops
  (q) edge[loop, in=180, out=240, looseness=8]  node[below, xshift=0pt, yshift=-6pt]  {$x_1 = 1$ \\ $\resetClock{x_1}$} (q)
  
  (q) edge[loop, in=90, out=150, looseness=8] node[right, xshift=21pt, yshift=0pt] {$x_2 = 2$ \\ $\resetClock{x_2}$} (q)
  
  (q) edge[loop, in=300, out=0, looseness=8] node[right, xshift=1pt, yshift=5pt] {$x_n = n$ \\ $\resetClock{x_n}$} (q)
  
  (q) edge node[right, yshift=-13pt] {$x_1 = \cdots = x_n = 0$ \\ $\land \; y \geq 1$} (goal);

  %\draw[red, thick, dashed] (current bounding box.south west) rectangle (current bounding box.north east);
\end{tikzpicture}
%\vspace{-17pt}
\caption{\flower{}. $q_0$ is initial.}
\label{fig:flower_main_text}
\end{wrapfigure}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/forward_reachability.tex <==
\input{Implementation_and_Experimental_Evaluation/figures/flower}
We compared \toolname{} against Uppaal 5.0 and TChecker (commit d711ace) in forward reachability\footnote{To ensure a fair comparison, symmetry reduction was disabled in both \toolname{} and Uppaal; notably, this optimization cannot be manually controlled in TChecker.}.
The benchmarks \Red{(adjusted to ensure compatibility across all tools)} come from publicly available repositories, published literature, or manually crafted when required.
If possible, the reachability queries match those of the original benchmarks; 
otherwise, they have been adapted to fit the capabilities of the tools.
%(\emph{e.g.}, TChecker only supports reachability via labelled locations).
%The original benchmarks have also been.
%(\emph{e.g.}, boolean variables were translated into integers, as boolean types are not yet supported by \toolname{}), and converted into the appropriate input formats.
%All experiments used \ac{dfs} exploration.
Uppaal was run with standard DBM without memory optimizations, TChecker was configured with the \texttt{covreach} flag to match the algorithm used in Uppaal.
%Symmetry reduction was disabled for both \toolname{} and Uppaal (it cannot be controlled in TChecker).
%
Experiments were conducted on a MacBook Pro equipped with an M3 chip and 24 GB of RAM.

In the following, tables report \ac{vt}, \ac{et}, memory (Mem, representing the Maximum Resident Set Size), and the number of stored regions and states.
\Red{\ac{et} measures the time elapsed between issuing a verification command and receiving the result from a tool.}
Timings are in seconds, memory in MB.
The size of a network is denoted by $K$ (for \flower{}, $K$ indicates the number of clocks).
All values are averages over five runs, with a timeout of 600 s set on \ac{et}.
Timeouts are reported as TO, $\varepsilon$ denotes times below 0.001 s, and out-of-memory events are denoted by OOM.
Bold cells indicate the fastest \ac{vt} (on ties, the fastest \ac{et}).
KO indicates that an error occurred during verification.
The complete benchmark suite is in the Appendix, \autoref{app:complete_experimental_evaluation}.



\textbf{\ac{ta} with punctual guards}~Region-based abstractions can outperform zone-based approaches when \acp{ta} are \emph{closed}, \emph{i.e.}, contain only non-strict guards.
This is particularly evident when guards are \emph{punctual}, \emph{i.e.}, restricted to equality constraints.
%
The \flower{} \ac{ta}~\cite{J_rgensen_2012} depicted in \autoref{fig:flower_main_text}, which is also used in our evaluation of backward reachability, satisfies these requirements.
It consists of two locations: $q_0$ (which is initial) and $\mathit{Goal}$, and it features $n + 1$ clocks, denoted by $x_1, \dots, x_n, y$.
The guards over clocks $x_i$ are punctual; the guard on $y$ is non-strict. 
Since $y$ is never reset, the behavior of \flower{} is equivalent to a model featuring only punctual guards.
To reach $\mathit{Goal}$, all clocks $x_i$ must simultaneously be exactly zero, while $y$ must satisfy $y \ge 1$.
Specifically, when transitioning to $\mathit{Goal}$, $y$ must be equal to the least common multiple of $1, 2, \dots, n$.
%
Similar behavior is shown in the additional examples reported in \autoref{tab:punctual}: these are networks of \ac{ta} with only punctual guards.
In all these experiments, punctual guards force zones to be repeatedly and finely split, as reflected by the large number of states shown in \autoref{tab:punctual}.
The results indicate that Uppaal and TChecker experience a substantial decrease in performance when $K \ge 8$.

\input{Implementation_and_Experimental_Evaluation/Benchmark_Tables/punctual_guards}



\textbf{Closed \ac{ta}}~Two networks of closed \acp{ta} were adapted from the benchmarks available on~\cite{tapaal2025}:
\medical{} models medical checks for patients, while \mpeg{} models the homonymous compression standard, where compression leverages a given number of bidirectional frames (BFrames).
Since \toolname{} does not currently support broadcast channels, these models were rewritten into equivalent versions that use only point-to-point channels.
The results in \autoref{tab:closed} reveal a high number of stored states.
This indicates that these models restrict the evolution of clocks in a way that forces zones to be repeatedly and finely split, thus pushing these models into a category where zone-based abstractions exhibit poor performance, a phenomenon already demonstrated in the above experiments (see \autoref{tab:punctual}).
Furthermore, both Uppaal and TChecker exhibit an unexpectedly high verification time in \medical{}. 
This indicates that the dominant cost in this benchmark originates from zone manipulation, whose operations may have quadratic or cubic complexity in the number of clocks~\cite{J_rgensen_2012}. 
Region-based analysis avoids this overhead, as its fundamental operations have linear complexity in the number of clocks.
Interestingly, TChecker aborted execution on the largest instances of \medical{} raising the error: \emph{"ERROR: value out of bounds"}.

\input{Implementation_and_Experimental_Evaluation/Benchmark_Tables/closed_ta}



\textbf{Large constants}~When constants are large, zones are still preferable.
%\todoAM{}{Magari dire anche che i vincoli in questi automi sono anche strict (vedere quali)}
%\todoAM{}{vedere se riferirsi a zone o dbm e usare quell in tutto il paper}
\autoref{tab:constants} reports results from two real-world case studies: the Carrier Sense Multiple Access / Collision Detection protocol (\csma{})~\cite{kiviriga2021randomized} and \pagerank{}~\cite{Baresi2020}, a mechanism used to prioritize Web keyword search results.
The latter is presented in two variants: in the first, the last two digits of the original constants were truncated, while the second uses the full constants.
The largest constant in \csma{} is 808, whereas in \pagerank{} they are 101 (truncated) and 10162 (full).

\input{Implementation_and_Experimental_Evaluation/Benchmark_Tables/big_constants}



\textbf{Safety properties}~When safety properties must be verified using forward reachability, \toolname{} requires to explore the entire reachable state space.
\autoref{tab:safety} reports the results for the Fischer mutual exclusion protocol~\cite{uppaalSite}.
The verified property specifies that two given processes must never be in the critical section simultaneously.
\Red{In the reminder of this section, we demonstrate that backward reachability may enhance the verification of safety properties by exploring only a restricted subset of the state space, potentially avoiding out-of-memory events.}

\input{Implementation_and_Experimental_Evaluation/Benchmark_Tables/full_state_space}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/implementation_and_experimental_evaluation.tex <==
This section introduces \toolname{} along with a detailed empirical evaluation of its forward and backward reachability algorithms.
To express reachability queries, we use the standard Computation Tree Logic formula $\exists \Diamond ( \varphi )$, meaning that there exists a path in the state space in which $\varphi$ eventually holds true.
%\todoAM{}{I secondi li riportiamo come 50s o 50 s?}

\subsection{The \textnormal{\toolname{}} library}
\input{Implementation_and_Experimental_Evaluation/tarzan}

\subsection{Forward reachability benchmarks}
\input{Implementation_and_Experimental_Evaluation/forward_reachability}

\subsection{Backward reachability analysis with \textnormal{\toolname{}}}
\input{Implementation_and_Experimental_Evaluation/backward_reachability}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Implementation_and_Experimental_Evaluation/tarzan.tex <==
\toolname{} is a C\texttt{++}20 library for performing forward and backward reachability analysis of \ac{ta} and networks of \ac{ta}, using either \ac{bfs} or \ac{dfs} state space exploration.
\toolname{} supports shared integer variables (specified by using general arithmetic expressions), urgent locations, and invariants. 
The semantics of both invariants and networks in \toolname{} follows those of Uppaal~\cite{Bengtsson2004}.
Support for networks of \ac{ta} and integer variables in backward reachability is currently under development.
Successors and predecessors algorithms were revised to allow each clock to have its own maximum constant.

\toolname{} accepts .txt input files, parsed using the Boost Spirit X3 library, containing a \ac{ta} representation written in a domain-specific language called \emph{Liana}.
Each file represents a single \ac{ta}; a network of \ac{ta} is defined using multiple files.

\textbf{Networks of \ac{ta}}~A \emph{network} of size $n$ is the parallel composition of $n$ individual \ac{ta}~\cite[Chapter 9]{Baier}.
Given $n$ regions $\reg_1, \dots, \reg_n$, each corresponding to a \ac{ta} $\aut_1, \dots, \aut_n$ in the network, a \emph{network region} $\overline{\reg}$ is defined as $\overline{\reg} := \{ \reg_1, \dots, \reg_n \}$. 
To compute both immediate delay and discrete successors of $\overline{\reg}$, \toolname{} 
%applies the respective successor algorithms to individual regions within $\overline{\reg}$;
%In particular, the immediate delay successor of $\overline{\reg}$ is obtained by computing the immediate delay successor of each $\reg_i \in \overline{\reg}$, whereas the discrete successors of $\overline{\reg}$ are determined from the discrete successors of the regions corresponding to the transitions that fire in the network.
{relies on specialized data structures that generalize the applicability of the algorithms originally developed for individual regions to network regions.
These data structures ensure the correctness of on-the-fly immediate delay and discrete successors computation across the Cartesian product of $\aut_1, \dots, \aut_n$.
In particular, a C\texttt{++} double-ended queue maintains the relative ordering of the fractional parts of all clocks within $\overline{\reg}$, partitioning these clocks into ordered equivalence classes.
This ordering captures the evolution over time of all clocks within $\overline{\reg}$, including which clocks will exit the unit (possibly becoming unbounded), reach the next unit, or be reset.
Furthermore, a C\texttt{++} set identifies the regions in $\overline{\reg}$ that are of class $\ca$ or $\cc$.
Since the generalized algorithms for network regions operate by applying the successors algorithms to a subset of individual regions in $\overline{\reg}$, this classification is essential for computing immediate delay successors; indeed, regions of class $\ca$ or  $\cc$ contain clocks that will exit the unit; hence, their immediate delay successors must be computed prior to those of regions of class $\cb$.}
%For instance, consider a network region $\overline{\reg'} = \{ \reg_1, \reg_2 \}$ such that $X_{\reg_1} = \{x, y, z\}$ and $X_{\reg_2} = \{w, t\}$.
%Let $v_1$ and $v_2$ be the clock valuations of $\reg_1$ and $\reg_2$, respectively, and assume that $\frc(v_1(y)) = \frc(v_1(z)) = \frc(v_2(w)) < \frc(v_1(x)) = \frc(v_2(t))$.
%Then, the corresponding deque for $\overline{\reg'}$ is $[\{x,t\}, \{y, z, w\}]$, where clocks with the smallest fractional part occupy the head of the deque and those with the largest fractional part occupy the tail.}
%
%
%The semantics of networks in \toolname{} follow those of Uppaal~\cite{Bengtsson2004}. 
%In particular, for any pair of \ac{ta} $(\aut_i, \aut_j)$ such that $(\reg_i, \reg_j) \in \overline{\reg}$, their set of actions may include \emph{synchronizing} actions, \emph{i.e.}, an \emph{output action} $a! \in \act_i$ and a corresponding \emph{input action} $a? \in \act_j$. 
%When a synchronizing action occurs, both transitions in $\aut_i$ and $\aut_j$ must be taken simultaneously.
%To prevent inconsistencies when updating shared integer variables during a synchronizing transition, specifically, when one \ac{ta} updates a variable that the other reads, we enforce that the transition corresponding to the output action fires before the transition corresponding to the input action.
%In other words, the discrete successor of $\reg_i$ $(a!)$ is computed before the discrete successor of $\reg_j$ $(a?)$.

%\textbf{Operational workflow}~\toolname{} accepts .txt input files containing a \ac{ta} description written in a \ac{dsl} called \emph{Liana}.
%Each file represents a single \ac{ta}; a network of \ac{ta} is defined using multiple files.
%\toolname{} uses the Boost Spirit X3 parser to generate a C\texttt{++} representation of the \ac{ta} defined in Liana. 
%Once parsing is completed, users can specify whether to perform a forward or backward reachability analysis.
%Currently, reachability queries can predicate over locations, clock values, and shared integer variables. 
%Queries are directly specified by passing the appropriate parameters to the \toolname{} API.

\textbf{Implementation considerations}~Since the focus of this paper is the implementation of algorithms using the new representation of \autoref{eq:region}, most optimizations are deferred to future work.
Currently, \toolname{} does not implement any optimizations for state space exploration, except for symmetry reduction~\cite{symmspin}.
Memory compression optimizations are not implemented either.
The algorithms also suffer when computing delay successors (predecessors), as these computations require generating a sequence of immediate delay successors (predecessors).
This limitation could be mitigated by implementing the optimization described in \autoref{sec:delay_and_discrete_predecessors} for delay predecessors (which can be adapted for delay successors as well).
\Red{Furthermore, since \toolname{} only performs reachability analysis, proving that a region is unreachable going forward requires exploring the entire reachable state space.}
\Red{Due to the aforementioned limitations, a \ac{bfs} exploration must visit all delay successors (predecessors) before visiting discrete successors (predecessors), which is typically unnecessary and increases the verification time.
For this reason, unless stated otherwise, all experiments follow a \ac{dfs} strategy.}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Introduction/introduction.tex <==
Formally verifying the behavioral correctness of real-time systems (also including distributed systems) is essential 
for ensuring that critical properties hold.
Since their introduction, \acp{ta} have become one of the most widely adopted formalisms for modeling and analyzing such systems~\cite{distributed2,distributed}.

A key challenge in the verification of \ac{ta} is their infinite state space, addressed by the \emph{region}~\cite{ALURDILL} abstraction, which provides a finite representation enabling algorithmic verification. Alternatives include \emph{Binary Decision Diagrams}~\cite{Wang2004} and \emph{zones}~\cite{HENZINGER1994193}, the latter requiring \emph{normalization} for state space finiteness~\cite{Bouyer2004}. 
Zones, typically implemented using \emph{\acp{dbm}}~\cite{DBM}, are widely used in tools such as Uppaal~\cite{UppaalTutorial}, TChecker~\cite{tcheckerpaper}, Kronos~\cite{KRONOS}, and Synthia~\cite{SYNTHIA}.

%A major challenge in the formal verification of \acp{ta} is the inherently infinite nature of their state space.
%To overcome this issue, the \emph{region} abstraction was introduced, providing a finite representation that enables algorithmic verification.
%Alternative abstractions of \ac{ta} have also been proposed, such as \emph{\acp{bdd}}~\cite{Wang2004} and \emph{zones}~\cite{HENZINGER1994193} (the latter requiring 	\emph{normalization} to ensure a finite-state abstraction of \acp{ta}~\cite{Bouyer2004}).
%Zones, in particular, have become the de facto standard in many practical tools (such as Uppaal~\cite{UppaalTutorial}, tChecker~\cite{tcheckerpaper}, Kronos~\cite{KRONOS}, and Synthia~\cite{SYNTHIA}), as they can be efficiently represented and manipulated using the \emph{\ac{dbm}} data structure~\cite{DBM}.

%Despite their popularity and practical efficiency,
%%, particularly when used in on-the-fly algorithms, 
%\acp{dbm} and \ac{dbm}-based zone representations still exhibit several shortcomings.
\Red{Zones have shown to be highly efficient in practice and, over the last decades, have become the de facto standard for the formal verification of \acp{ta}, although they have well-known limitations~\cite{quantitativebouyer,Lehmann2023,Yovine1998}.
%their success is partly due to a fundamental limitation of discretized abstractions, which suffer from severe state space explosion when the underlying \ac{ta} features large constants or many clocks. 
%Consequently, no region-based verification tool or reusable library is, to the best of our knowledge, currently available.
Yet, prior work has demonstrated that for the class of \emph{closed} \acp{ta}, \emph{i.e.}, \ac{ta} containing only non-strict guards, region-based abstractions may outperform state-of-the-art zone-based tools~\cite{J_rgensen_2012}.}

\Red{The promising performance of region-based abstractions on appropriate subclasses of \acp{ta} motivated the development of \toolname{} (Timed Automata Region and Zone library for real-time systems ANalysis)~\cite{tarzan2025}, a C\texttt{++}20 library designed to support and complement state-of-the-art zone-based tools for the formal verification of \acp{ta}.}
Currently, \toolname{} supports only region-based reachability of \ac{ta}; optimizations leveraging zones are deferred to future work.
%The region abstraction used in \toolname{} refines the classical abstraction by tracking the order in which clocks become unbounded.
The implementation of backward reachability algorithms enables the extension of \toolname{} to domains in which backward analysis is essential, such as Timed Games~\cite{PnueliTG}.

\Red{When compared against zone-based state-of-the-art tools including Uppaal and TChecker, \toolname{} exhibits superior performance on \ac{ta} and networks of \ac{ta} featuring \emph{punctual} guards, \emph{i.e.}, guards with equality constraints, and on closed \ac{ta}, even with large constants or many clocks.
However, the size of constants remains a significant bottleneck in other classes of \ac{ta} (\emph{e.g.}, zones excel in \ac{ta} with strict guards).
Moreover, since \toolname{} only supports reachability analysis, using forward reachability to verify safety properties for unreachable regions requires exploring the entire reachable state space.
We show in this paper that backward reachability can enhance the verification of safety properties.}

% VEDERE SE METTERE QUESTO PARAGRAFO SOTTO
%Despite their practical efficiency, \ac{dbm}-based zones have limitations. 
%After normalization, they often yield more zones than regions~\cite{quantitativebouyer}, though on-the-fly algorithms rarely explore the full zone graph. 
%Standard \ac{dbm} operations provide limited control over individual entries, and \ac{dbm} sequences may grow uncontrollably~\cite{Lehmann2023}. 
%Moreover, because \acp{dbm} compactly represent sets of adjacent regions, they perform poorly when encoding non-contiguous region sets~\cite{Yovine1998}.

%Zones pose significant challenges when solving \emph{Timed Games}~\cite{PnueliTG}, \emph{i.e.}, games on graphs~\cite{GoG} played over \acp{ta}, where the goal is to \Red{synthesize} 
%\todoAM{}{compute o synthesize?}
%winning strategies that typically capture reachability or safety objectives. The issues arise because zones may over-approximate the reachable state space, potentially leading to incorrect synthesis or misclassification of strategies.
%\Red{To address these shortcomings, one may use costly preprocessing techniques~\cite{ontheflycontroller} or ad-hoc, on-the-fly algorithms that refine the zone abstraction~\cite{efficientonthefly}.
%Although effective in practice, these algorithms may have higher theoretical complexity than region-based approaches.}
%To address these shortcomings, one may resort to costly preprocessing techniques~\cite{ontheflycontroller}, or to ad-hoc, on-the-fly algorithms that refine the zone abstraction~\cite{efficientonthefly}. While these algorithms may perform well in practice, their theoretical complexity can be higher than that of region-based approaches.

%The above limitations highlight that the region abstraction remains a compelling alternative to zones, especially in problems requiring a fine-grained analysis, provided that an appropriate representation of regions is available, including mechanisms to handle unbounded clocks.

\textbf{Related works}~Abstractions closely related to regions have already been proposed to better capture the semantics of \ac{ta}.
In~\cite{TowardsUnbounded}, regions are encoded as Boolean formulae via discrete interpretations.
The \emph{slot-based} abstraction proposed in~\cite{2024parameterized} groups regions by time using integer-bounded intervals over a global clock.
A data structure, called \emph{time-dart}, is introduced in~\cite{J_rgensen_2012} to compactly encode configurations of \ac{ta} and their time successors without explicit enumeration.
In~\cite{Bouyer2008}, regions of bounded \ac{ta} are represented as tuples combining integer clock values and a partition of clocks that reflects the ordering of their fractional parts.
The region abstraction is extended in~\cite{math12244008} to \emph{durational-action} \ac{ta}.
%None of these abstractions tracks the order in which clocks become unbounded.

To the best of our knowledge, no region-based library for \acp{ta} verification, nor any libraries or tools based on the aforementioned abstractions, currently exist. 
Consequently, we compare \toolname{} against the state-of-the-art tools Uppaal and TChecker.
Existing libraries that explicitly support the analysis of \ac{ta} using \ac{dbm}-based zone representations include~\cite{PyDBM,UDBM}.
Other libraries offer more general polyhedral abstractions beyond zones, such as those provided by~\cite{apron,PPL}.

\textbf{Contributions}~The main contribution of this work is two-fold:
(i) we first introduce a refined region representation that tracks the order in which clocks become unbounded.
While this representation may increase the total number of regions by inducing a finer partitioning of the state space, a major advantage is that it guarantees at most three immediate delay predecessors for any region;
(ii) building on this new representation, we develop and implement algorithms in \toolname{} for computing delay and discrete successors and predecessors of regions.
\Red{Existing tools may integrate \toolname{} to enhance their verification capabilities.}
%forward and backward reachability analysis of \ac{ta}.

This paper is organized as follows:
\autoref{sec:theoretical_background} introduces the necessary theoretical background.
\autoref{sec:data_structure} presents the proposed new region representation, from which a classification of regions is derived.
\autoref{sec:delay_and_discrete_predecessors} details the algorithms (and their pseudocode) to compute discrete successors and immediate delay predecessors of regions using this representation.
\autoref{sec:implementation_and_experimental_evaluation} presents an overview of \toolname{} and provides an empirical evaluation of forward and backward reachability.
\autoref{sec:conclusion} concludes and outlines future developments.
An appendix provides additional algorithms, proofs, and full experimental results.

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/Theoretical_Background/theoretical_background.tex <==
The timing behavior of real-time systems is naturally modeled by the formalism of TA, which is obtained by extending classical finite-state automata with real-valued clocks. In the following, we use the term action to refer to the events that a real-time system can exhibit.
\acp{ta} are defined as follows~\cite{ALURDILL}:

\begin{definition}%[\acl{ta}]
\label{def:tadef}
{A \emph{\acl{ta}} $\aut$ is a tuple $\aut = (\act, Q, Q_{0}, \ackc, T, \invariant)$, where
$\act$ is a finite set of actions,
$Q$ is a finite set of locations,
$Q_{0} \subseteq Q$ is a set of initial locations,
$\ackc$ is a finite set of clocks,
$T \subseteq Q \times \act \times \Gamma(\ackc) \times 2^{\ackc} \times Q$ is a transition relation, and
$\invariant : Q \rightarrow \Gamma(\ackc)$ is an invariant-assignment function.}
\end{definition}

Let $\aut$ be a \ac{ta}.
Clocks are special variables that can only be reset or compared against non-negative integer constants. 
The value of all clocks is initialized to zero and grows with derivative 1 until a reset occurs.
When a clock is reset, its value becomes zero; after a reset, it starts increasing again. 
$\Gamma(\ackc)$ is the set of \emph{clock guards}, \emph{i.e.}, conditions
{over clocks} that must be satisfied for a transition to fire.
Clock guards are defined by the following grammar: 
$\gamma := 
\xi
\; | \;
\gamma \land \gamma$, 
where 
$\xi := 
x \sim c$ 
is a \emph{clock constraint}, $x \in \ackc$, $c \in \mathbb{N}$, and $\sim \; \in \{ \le, <, =, >, \ge \}$.
We write $\xi \in \gamma$ to indicate that the clock constraint $\xi$ occurs within the guard $\gamma$.
For instance, if $\gamma := x_1 < c \land x_2 \ge c$, then $\xi_1 := x_1 < c$ and $\xi_2 := x_2 \ge c$, where $\xi_1, \xi_2 \in \gamma$. 
%For readability, standard logical equivalences are applied in clock constraints, \emph{e.g.}, $\neg(x < c) \equiv x \ge c$.
The powerset $2^{\ackc}$ indicates that a transition may reset a {subset} of the clocks.
We denote by $\cmax \in \mathbb{N}$ the maximum constant appearing in $\aut$ and assume, without loss of generality, that it is the same for all clocks of $\aut$.

A pair $(q, v)$ is a \emph{configuration} of a \ac{ta} $\aut$, where $q \in Q$ and $v : \ackc \rightarrow \mathbb{R}_{\ge 0}$ is a \emph{clock valuation} function.
We denote by $\eval$ the set of all clock valuations of $\aut$.
Given a subset $Y \subseteq \ackc$ of clocks, we denote by $\valZ$ the clock valuation defined as $\valZ(x) = 0$ if $x \in Y$ and $\valZ(x) = v(x)$ otherwise.
%\todoMR{}{siccome la clock valuation è $\valZ$ la $(x)$ andrebbe dopo, $\valZ(x)$.
%AM: sistemato}
Given a constant $\delta \in \mathbb{R}_{\ge 0}$ and a clock $x \in \ackc$, the value $(v + \delta)(x)$ is defined as $v(x) + \delta.$

{The \emph{transition system} $\transta = (S, \act \cup \mathbb{R}_{\ge 0}, I, \hookrightarrow)$ captures the semantics of a \ac{ta} $\aut$, where 
$S = Q \times \eval$,
$I = \{ (q, v) \; \vert \; q \in Q_0 \land \forall x \in \ackc : v(x) = 0 \}$, and 
$\hookrightarrow$ is the transition relation containing:
(i) \emph{discrete} transitions $((q,v), a, (q',v'))$ if there exists a transition $(q, a, \gamma, Y, q') \in T$ in $\aut$ such that $v$ satisfies both $\gamma$ and $\invariant(q)$, and $v'(x) = \valZ(x)$ satisfies $\invariant(q')$, where $a \in \act$, for all $x \in \ackc$, and
(ii) \emph{delay} transitions $((q,v), \delta, (q,v'))$ if there exists a constant $\delta \in \mathbb{R}_{\ge 0}$ such that $v'(x) = (v + \delta)(x)$ satisfies $\invariant(q)$, for all $x \in \ackc$.
A full description of the standard transition system semantics of \ac{ta} is covered in~\cite[Chapter 9]{Baier}.}

The infinite state space of \acp{ta} can be conveniently analyzed by resorting to a finite abstraction, known as the \emph{region} abstraction~\cite{ALURDILL}.
For any real number $m \in \mathbb{R}$, we denote its integral and fractional parts by $\lrf{m}$ and $\frc(m)$, respectively.

\begin{definition}[Clock equivalence relation]
\label{def:clock_equivalence}
Let $\aut\! =\! (\act, Q, Q_{0}, \ackc, T, \invariant)$ be a \ac{ta}.
Two clock valuations $v, v' \in \eval$ are called \emph{clock-equivalent}, denoted by $v \cong v'$, if, and only if, it either holds that:
\emph{(i)} $v(x) > \cmax$ and $v'(x) > \cmax$, for all $x \in \ackc$, or 
\emph{(ii)} 
for any $x, y \in \ackc$, with $v(x), v'(x) \le \cmax$ and $v(y), v'(y) \le \cmax$,
it holds that:
\emph{(ii$_a$)} $\lrf{v(x)} = \lrf{v'(x)}$ and $\frc(v(x)) = 0$ $\Leftrightarrow$ $\frc(v'(x)) = 0$, and
\emph{(ii$_b$)} $\frc(v(x)) \sim \frc(v(y))$ $\Leftrightarrow$ $\frc(v'(x)) \sim \frc(v'(y))$, where $\sim \; \in \{<, =\}$.
\end{definition}

\begin{definition}[Region]
Let $\aut$ be a \ac{ta} and $s = ( q, v )$ be a configuration of $\aut$.
The \emph{clock region} $[v]$ of $v \in \eval$ is the set of all clock valuations equivalent to $v$ under the relation of \autoref{def:clock_equivalence}.
%, where $q \in Q$ and $v \in \eval$,
The \emph{state region} $[s]$ of $s$ is: $[s] = ( q, [v] ) = \{ ( q, v' ) \mid v' \in [v] \}$;
$[s]$ is \emph{initial} iff $q \in Q_0$ and $\forall v' \in [v], \forall x \in \ackc : v'(x) = 0$.
\end{definition}

In the remainder of this work, we focus on state regions, referred to simply as \emph{regions}.
\Red{Let $\aut$ be a \ac{ta} and $[s] = ( q, [v] )$ a region of $\aut$.
A region $[s'] = ( q', [v'] )$ is an \emph{immediate delay successor} of $[s]$ if either:
(i) $q = q' \land [v] = [v']$ and, for all $\bar{v} \in [v]$ and $x \in \ackc$, $\bar{v}(x) > \cmax$, or
(ii) $q = q' \land [v] \neq [v']$ and 
for all $\bar{v} \in [v]$ 
there exists $\delta \in \mathbb{R}_{> 0}$
such that $\bar{v} + \delta \in [v'] 
\land 
\forall \; 0 \le \delta' \le \delta : \bar{v} + \delta' \in ([v] \cup [v'])$.
A region $[s']$ is a \emph{delay successor} of $[s]$ if there exists a finite sequence of regions $[s_0], [s_1], \dots, [s_n]$ such that $[s_0] = [s]$, $[s_n] = [s']$, and each $[s_{i + 1}]$ is an immediate delay successor of $[s_i]$, for $0 \le i < n$.
A region $[s']$ is a \emph{discrete successor} of $[s]$ if $[v'] = [\valZ]$, where $Y \subseteq \ackc$ is the subset of clocks reset over the discrete transition from $[s]$ to $[s']$.
Symmetric definitions can be given for \emph{immediate delay predecessors}, \emph{delay predecessors}, and \emph{discrete predecessors}.}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/comments.tex <==
\large{\textbf{COMMENTS}}

\begin{enumerate}
    \item LINEA 192 (ultimo paragrafo prima della sezione sui delay predecessor)

    Qui ogni volta si potrebbe tornare indietro alternando B e C, però in questo caso dovremmo ruotare ogni volta i clock bounded per come sono definiti gli spostamenti tra classi, occorre calcolare nel dettaglio quanti passi della computazione occorre fare. Vedere esempio grafico sugli appunti per capire il meccanismo di rotazione, poi calcolare quanti passi effettivamente occorre fare, tenend conto che il predecessore di una regione C è unico mentre di una regione B sono 3 (verificare che effettivamente sono sempre 3 ad ogni passo). Intuitivmente qui i passi da effettuare dovrebbero essere pari a $(\cmax - 1) \cdot p$ (vedere poi di quale p si tratta o se è ininfluente la scelta tra quello di $\regb$ oppure $\regc$.)
\end{enumerate}

==> Tracking_Clock_Unboundedness__A_Refined_Region_Representation_for_Timed_Automata/macros.tex <==
% --- PACKAGES --- %

\usepackage[textwidth=3.5cm,textsize=footnotesize]{todonotes}
%\usepackage[textwidth=3.5cm,textsize=footnotesize,disable]{todonotes}
\newcommand{\todoPL}[2]{\todo[color=yellow!50,#1]{\textbf{PL:}#2}}
\newcommand{\todoAM}[2]{\todo[color=red!50,#1]{\textbf{AM:}#2}}
\newcommand{\todoMR}[2]{\todo[color=green!50,#1]{\textbf{MR:}#2}}
\setlength{\marginparwidth}{4cm}

\newcommand{\Red}[1]{{\color{black}#1}}
%\newcommand{\Red}[1]{{\color{red}#1}}
\newcommand{\Blue}[1]{{\color{blue}#1}}


\newcommand{\resetClock}[1]{\mathbf{#1 \boldsymbol{:=} 0}}




\newcommand{\reg}{\mathcal{R}}
\newcommand{\breg}{\boldsymbol{R}}

\newcommand{\rega}{\mathcal{R}_{\ca}}
\newcommand{\regb}{\mathcal{R}_{\cb}}
\newcommand{\regc}{\mathcal{R}_{\cc}}
\newcommand{\regu}{\mathcal{R}_{\cu}}

\newcommand{\ca}{Z}
\newcommand{\cb}{P}
\newcommand{\cc}{M}
\newcommand{\cu}{U}

\newcommand{\loc}{q}

\newcommand{\ta}{\mathcal{A}}

\newcommand{\cmax}{c_m}

\newcommand{\algx}{\mathcal{X}}

\newcommand{\dpred}{\mathit{DP}}


% --- THEORETICAL BACKGROUND --- %

\newcommand{\act}{\mathit{Act}}

\newcommand{\aut}{\mathcal{A}}

\newcommand{\transta}{\mathit{TS}(\aut)}

\newcommand{\ackc}{X_{\aut}}
\newcommand{\ackcp}{X_{\aut'}}

\newcommand{\cckc}{X_{\winCond}}

\newcommand{\valXZ}{v(x)[Y \leftarrow 0]}

\newcommand{\valZ}{v[Y \leftarrow 0]}

\newcommand{\AP}{\mathit{AP}}

\newcommand{\eval}{\mathit{Eval}_{\aut}}

\newcommand{\frc}{\mathit{fr}}

\newcommand{\lrf}[1]{\lfloor #1 \rfloor}

\newcommand{\rtsstate}{\mathcal{S}}

\newcommand{\Next}{\vcenter{\hbox{$\bigcirc$}}}
%\medcircle
%\newcommand{\Next}{\mathbf{X}}

\newcommand{\Prev}{\vcenter{\hbox{\scalebox{1.375}{$\ominus$}}}}
%\ominus
%\newcommand{\Prev}{\mathbf{Y}}

\newcommand{\Until}{\mathbf{U}}

\newcommand{\Since}{\mathbf{S}}

\newcommand{\Globally}{\Box}
%\newcommand{\Globally}{\mathbf{G}}

\newcommand{\Eventually}{\Diamond}
%\newcommand{\Eventually}{\mathbf{F}}

\newcommand{\RTSA}{\mathcal{R}_{\mathcal{A}}}

\newcommand{\res}{\mathit{res}}

\newcommand{\ccstr}{\xi}

\newcommand{\bareg}{\overline{\reg}}

\newcommand{\allclocks}[1]{\mathbf{X}_{#1}}

\newcommand{\rtsarrow}{\rightsquigarrow}

\newcommand{\invariant}{\mathit{Inv}}



% ----- REGION DATA STRUCTURE ----- %
\newcommand{\lidx}{\boldsymbol{\ell}}
\newcommand{\ridx}{\mathfrak{r}}



% ----- IMPLEMENTATION ----- %
\newcommand{\toolname}{\textsc{Tarzan}}

\newcommand{\boolea}{\texttt{boolean}}
\newcommand{\flower}{\texttt{flower}}
\newcommand{\gates}{\texttt{gates}}
\newcommand{\ring}{\texttt{ring}}
\newcommand{\exSITH}{\texttt{exSITH}}
\newcommand{\csma}{\texttt{CSMA/CD}}
\newcommand{\pagerank}{\texttt{pagerank}}
\newcommand{\fischer}{\texttt{fischer}}
\newcommand{\medical}{\texttt{medicalWorkflow}}
\newcommand{\mpeg}{\texttt{mpeg2}}
\newcommand{\lynch}{\texttt{lynch}}
\newcommand{\train}{\texttt{trainAHV93}}
\newcommand{\bridge}{\texttt{bridge}}
\newcommand{\latch}{\texttt{latch}}
\newcommand{\maler}{\texttt{maler}}
\newcommand{\rcp}{\texttt{rcp}}
\newcommand{\soldiers}{\texttt{soldiers}}
\newcommand{\srlatch}{\texttt{srLatch}}
\newcommand{\simple}{\texttt{simple}}
\newcommand{\andor}{\texttt{andOrOriginal}}


\acrodef{ta}[TA]{Timed Automaton}
\acrodefplural{ta}[TA]{Timed Automata}
\acrodef{tarena}[TAr]{Timed Arena}
\acrodefplural{tarena}[TArs]{Timed Arenas}
\acrodef{tg}[TG]{Timed Game}
\acrodefplural{tg}[TGs]{Timed Games}
\acrodef{ltl}[LTL]{Linear Temporal Logic}
\acrodef{cltloc}[CLTLoc]{Constraint Linear Temporal Logic over clocks}
\acrodef{cltl}[CLTL]{Constraint LTL}
\acrodef{ctl}[CTL]{Computation Tree Logic}
\acrodef{tctl}[TCTL]{Timed Computation Tree Logic}
\acrodef{tol}[TOL]{Timed Obstruction Logic}
\acrodef{rts}[RTS]{Region Transition System}
\acrodefplural{rts}[RTSs]{Region Transition Systems}
\acrodef{gba}[GBA]{Generalized Büchi Automaton}
\acrodefplural{gba}[GBA]{Generalized Büchi Automata}
\acrodef{dbm}[DBM]{Difference Bound Matrix}
\acrodefplural{dbm}[DBMs]{Difference Bound Matrices}
\acrodef{bdd}[BDD]{Binary Decision Diagram}
\acrodefplural{bdd}[BDDs]{Binary Decision Diagrams}

\acrodef{bfs}[BFS]{breadth-first}
\acrodef{dfs}[DFS]{depth-first}
\acrodef{tarzan}[TARZAN]{Timed Automata Region and Zone library for real-time systems ANalysis}
\acrodef{dsl}[DSL]{Domain-Specific Language}
\acrodef{vt}[VT]{Verification Time}
\acrodef{et}[ET]{Execution Time}

==> comments.tex <==
\large{\textbf{COMMENTS}}

\begin{enumerate}
    \item LINEA 192 (ultimo paragrafo prima della sezione sui delay predecessor)

    Qui ogni volta si potrebbe tornare indietro alternando B e C, però in questo caso dovremmo ruotare ogni volta i clock bounded per come sono definiti gli spostamenti tra classi, occorre calcolare nel dettaglio quanti passi della computazione occorre fare. Vedere esempio grafico sugli appunti per capire il meccanismo di rotazione, poi calcolare quanti passi effettivamente occorre fare, tenend conto che il predecessore di una regione C è unico mentre di una regione B sono 3 (verificare che effettivamente sono sempre 3 ad ogni passo). Intuitivmente qui i passi da effettuare dovrebbero essere pari a $(\cmax - 1) \cdot p$ (vedere poi di quale p si tratta o se è ininfluente la scelta tra quello di $\regb$ oppure $\regc$.)
\end{enumerate}
